CODIT: Code Editing with Tree-Based Neural Models

The way developers edit day-to-day code tends to be repetitive, often using existing code elements. Many researchers have tried to automate repetitive code changes by learning from specific change templates which are applied to limited scope. The advancement of deep neural networks and the availability of vast open-source evolutionary data opens up the possibility of automatically learning those templates from the wild. However, deep neural network based modeling for code changes and code in general introduces some specific problems that needs specific attention from research community. For instance, compared to natural language, source code vocabulary can be significantly larger. Further, good changes in code do not break its syntactic structure. Thus, deploying state-of-the-art neural network models without adapting the methods to the source code domain yields sub-optimal results. To this end, we propose a novel tree-based neural network system to model source code changes and learn code change patterns from the wild. Specifically, we propose a tree-based neural machine translation model to learn the probability distribution of changes in code. We realize our model with a change suggestion engine, CODIT, and train the model with more than 24k real-world changes and evaluate it on 5k patches. Our evaluation shows the effectiveness of CODITin learning and suggesting patches. CODIT can also learn specific bug fix pattern from bug fixing patches and can fix 25 bugs out of 80 bugs in Defects4J.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		$(name).out \
		psfig.aux \
		*.bbl \
		*.pdfsync \
		$(name).fdb_latexmk \
		$(name).fls \
		$(name).synctex.gz


#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> backups/approach.tex <==
\section{Implementation}
\label{sec:approach}

Using our tree2tree NMT model, we implement a source code suggestion tool, \tool. \tool learns source code changes from a pool of patches in the wild. Then, given a code fragment to modify, \tool predicts potential changes that are likely to take place in the similar context. We implemented \tool using theano on top of python2.7. 
This section elaborates \tool implementation, \ie our patch processing, training, and testing approaches in detail.

\noindent
\textbf{Patch Pre-processing.} 
As a first step of the training process, \tool takes a pool of patches as input and represent them in parse tree format. 
\tool works at method granularity. 
For a method patch $\Delta m$, \tool takes two versions of $m$: \mold and \mnew. 
%The edits are represented as a sequence of insertions, deletions, and updates. 
%Thus, a patch to $m$ is represented as $\Delta m = (e_o, e_1, . . . , e_n)$.
\tool uses GumTree, a tree-based code differencing tool~\cite{falleri2014fine}, to identify the edited AST nodes of the two versions. The edit operations are represented as insertion, deletion, and update of a node \wrt \mold.
 \tool then selects a minimal subtree 
 of each AST that captures all of its edited nodes. 
 %These subtrees, \pold and \pnew, represent the AST representation of the patches.  change tree \wrt to \mold. 
The number of nodes in \mold's AST is {\em edit size}. For example, in~\Cref{fig:motiv_pt}, ~\Red{red} nodes are identified as deleted nodes and~\Green{green} nodes are marked as added nodes. 

\tool further collects the edit context by including the nodes that connect the root of the method to the root of the changed tree. 
For example, in~\Cref{fig:motiv_pt}, it ignores the dotted sub-trees. 
In the process, \tool excludes any changes occurred in JavaDoc, comments, and constants. Finally, for each method pair, \tool gets a pair $(AST_{old}, AST_{new})$ where $AST_{old}$ is the original AST where change was applied, and $AST_{new}$ is the AST after the changes.


% That gives us the source change tree ($S_{TC}$). 
% The number of nodes in $S_{TC}$ is the change size ($C_{TC}$). 
% We have two parameters for collecting the dataset: i. $m_c$: maximum change size, and ii. $m_t$: maximum tree size. 

% To provide context to the model, we went further into the ancestor chain from the root of $S_{TC}$ all the way to root of $T_{sm}$ until the tree size exceeds a maximum threshold. 
% In the process, we excluded JavaDoc changes, changes in comments, and changes in strng and other constant values. Finally, for each method pair, we get a pair $(AST_b, AST_a)$ where $AST_b$ is the original AST, and $AST_a$ is the code after the changes.


%\sk{Baishakhi and Miltos: Please read this.   Changes in constant values are highly circumstantial and cannot be predicted accurately without concrete analysis of the project execution situation. This is not in the scope of this work and we leave the concretization of the constant values to augment our proposed approach as future research.} 

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=\textwidth]{images/ast-pt.png}
%     \caption{\textbf{\small AST and Parse Tree of the expression $\mathbf{z = x + y}$}}
%     \label{fig:ast-pt}
% \end{figure}



% \subsubsection{Parse Tree Generation}
% \label{subsubsec:parsetree-gen}
% \noindent
% \textit{(ii) Parse Tree Generation.}
\tool then converts the ASTs to the parse tree representation. 
In AST, non-terminals can hold values. 
% For example, in~\Cref{fig:ast-pt}, node $n_1$ and $n_2$ in the AST hold a values(`$=$' and `$+$') although they are non-terminals. 
For our model, we only want terminals to hold values so that they can form token sequences. Hence, \tool converts the AST to a parse tree representation. 
% pulling the value of a non-terminal as a terminal child of that non-terminal in appropriate position. In AST generated by GumTree, Java language constructs (such as `$;$', `$($', `$)$') are also encoded implicitly in the AST. We did not want that either. We searched in the source code for missing tokens and added those in appropriate positions as terminals. 
Thus, the final pair of parse trees representing a patch is ($PT_{old}, PT_{new}$). 
 
%\input{model.tex}

To train the model, we first sorted the patches of our dataset chronologically. Then, we took the first 75\% of the patches from each project as training, 
15\% as validation, and the rest 10\% as testing. This way of partitioning the data reflects how a developer would use a model in real life: a model trained on past patches will be used to predict future edits. 



\noindent
\textbf{Model Training.}
The objective of this step is to optimize the parameters of the network to maximize the probability estimation of~\Cref{eqn:a_t}. First, we used the cross-entropy loss as the objective function. However, in our preliminary experiment, we found that the quality of the generated code is not directly related to the loss. To mitigate this problem, we used BLEU score~\cite{papineni2002bleu}, a standard metric to evaluate translation models, as an alternate way of evaluating the trained model. We run the training model for a fixed amount of time ($n_{epoch}$). However, if the model performance (in terms of BLEU score) on validation data does not improve consecutively over a fixed number of steps ($valid_{patience}$), we stop training procedure and declare the best-resulting model as the target model. 


% To train the model described above, we first sorted the commits in out dataset based on the chronology. The motivation is, developer can train a model based on earlier changes only. Then developer can deploy a trained model subsequent changes. In line with that motivation, we divided our commits in every project in our dataset  in 2 parts. First 75\% commits are kept as train commits, next 10\% as validation commits, and rest 15\% are kept as testing commits. After that, we extract all the patches from train, validation, and test commit sets to train, validation and test data respectively.  In training, the objective is to optimize the parameters of the network to maximize probability estimation of equation~\ref{eqn:a_t}. We used cross-entropy loss based of this probability estimation as objective function. To optimize the parameters in the model, we used the Adam optimizer.  However, in our preliminary experiment, we found that, the quality of generated code is not directly related to the loss. To mitigate this problem, we used BLEU score~\cite{papineni2002bleu} as an alternative way of measuring the performance of trained model. We run the training model for a fixed amount of time ($n_{epoch}$). However, if the model performance (in terms of BLEU score) on validation data does not improve consecutively over a fixed number of steps ($valid_{patience}$), we stop training procedure and declare the best resulting model as the target model. Since throughout all $valid_{patience}$ training iteration, the model could produce better result on validation dataset, our decision for early stop is rational. We believe the model had reached optima. We used Adam optimizer to optimize the model. 

%\subsection{Testing and Deployment of the Model}
%\label{subsec:testing}
% \begin{algorithm}[htb]
%     \caption{Beam Search Algorithm for Inferring Changed Code. $x$ is the input code, $\mathscr{G}$ is the Grammar.}

% \SetAlgoLined
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \SetKwInOut{Return}{return}
% \underline{\textbf{Function beam-search($x$)}} \\
% \SetAlgoVlined
% \Input{$x$ - input code}
% \Output{$[y]$ - list of codes after changes}
%  $init\_state = Encoder(x)$\\
%  $root\_hyp = Hypothesis(init\_state)$\\
%  $all\_hyps = [root\_hyp]$\\
%  $completed\_hyps = []$\\
%  \For{i = 1 to max\_timestep}{
%       $new\_hyps = []$\\
%       \For{q in all\_hyps}{
%         \eIf{$q.n_f^t\text{ is non-terminal}$}{
%             \For{$rule \in \mathscr{G}$}{
%                 $q' = q.ApplyRule(rule)$\\
%                 $q'.score = q.score + rule.log\_prob$\\
%                 add $q'$ to new\_hyps\\
%             }
%         }{
%             \For{$v \in Vocab$}{
%                 $q' = q.InsertToken(v)$\\
%                 $q'.score = q.score + v.log\_prob$\\
%                 \eIf{$q'.isCompleted()$}{
%                     add $q'$ to completed\_hyps\\
%                 }{
%                     add $q'$ to new\_hyps\\
%                 }
%             }
%         }
%       }
%       $\text{sort new\_hyps based on score}$\\
%       $\text{all\_hyps = top k Hypotheses fron new\_hyps}$\\
%   }
%  sort completed\_hyps based on score\\
%  \Return{top $K$ hypotheses from completed\_hyps}
%  \label{alg:inference}
% \end{algorithm}
\noindent
\textbf{Model Testing.}
To test the model and generate changes, we adopt a beam-search-based approach~\cite{reddy1977speech}\textemdash instead of generating one target tree, at each step of the decoder, we generate $K$ (partially generated-) trees. In beam search's terminology,
%we call every tree, either partially or completely generated, 
these are states/hypotheses.
At each time step, we pick the top $K$ partial expansions. Then, we explore all states by all possible expansions 
reachable from those $K$ states. If we find a state that is completed (\ie a state containing a complete tree), we exclude that hypothesis from further expansion. We then pick top $K$ incomplete hypotheses based on the score. We stop this process if max time step is reached or if there is no more incomplete hypothesis to be expanded. We then sort all completed hypotheses based on the probability score and  generate code from top $K$ hypotheses. Finally,  we generate $K$ different code fragments from $K$ different hypotheses. 
% The inference procedure is articulated in Algorithm~\ref{alg:inference}. 


==> backups/approach_back.tex <==
\section{Approach}
\label{sec:approach}
We formulate the change generation problem as a machine translation model. In machine translation, there are several methods for translating sentence/phrase from one language to another. Since all the languages does not follow the same grammar, the Neural Machine Translation (NMT) model learns the transformation pattern that makes a successful translation. NMT models are usually a cascade of an Encoder and a Decoder. The most common and successful NMT model is sequence-to-sequence (seq2seq) model~\cite{bahdanau2014neural}, where the input is treated as a sequence of tokens and encoded by a sequential encoder (\eg an LSTM) and the output is generated a stream of tokens (via a sequence decoder). In NMT literature, several improvements made over the base seq2seq model, such as attention and copying, that we also employ here.

\subsection{Data Collection}
\label{subsec:data-col}
\subsubsection{Collecting Raw Data}
We chose 60 different well-established projects from GitHub to train our model. These projects are from the TravisTorrent dataset~\cite{msr17challenge} and are moderately big projects with well-maintained code base. 
% The data collection procedures are described in subsequent sections. 
% \subsubsection{Collecting commits}
% \label{subsub:co,-commit}
For each project from the TravisTorrent dataset, we collected the revision history of the main branch. 
If a commit affects a Java file, we stored both the previous version ($f_{s}$) of the file and the version after commit ($f_{t}$). 
We then extracted method pairs from each file pair $(f_{s}, f_{t}$) into
$MP_{st}=\{(m_{s}^i, m_{t}^i)\}$ which is a list of changed method pairs from $(f_{s}, f_{t}$). 
Then, we pass a $MP_{st}$ to our change extractor.
We built our change extraction tool on top of GumTree code differencing tool~\cite{falleri2014fine}. 
For each pair, we get a set of edits ($E_{st}$) in source method AST ($T_{sm}$). 
The edit operations in AST are, i. insertion of a node, ii. deletion of a node, and iii. replacement of a node. 
We select the highest depth node from the source method AST that captures all the edits in $E_{st}$. 
That gives us the source change tree ($S_{TC}$). 
The number of nodes in $S_{TC}$ is the change size ($C_{TC}$). 
We have two parameters for collecting the dataset: i. $m_c$: maximum change size, and ii. $m_t$: maximum tree size. 
To provide context to the model, we went further into the ancestor chain from the root of $S_{TC}$ all the way to root of $T_{sm}$ until the tree size exceeds $m_t$. 
In the process, we excluded JavaDoc changes, changes in comments, and changes in strng and other constant values. \sk{Baishakhi and Miltos: Please read this.   Changes in constant values are highly circumstantial and cannot be predicted accurately without concrete analysis of the project execution situation. This is not in the scope of this work and we leave the concretization of the constant values to augment our proposed approach as future research.} Finally, for each method pair, we get a pair $(AST_b, AST_a)$ where $AST_b$ is the original AST, and $AST_a$ is the code after the changes

\subsubsection{Parse Tree Generation}
\label{subsubsec:parsetree-gen}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\textwidth]{images/ast-pt.png}
    \caption{\textbf{\small AST and Parse Tree of the expression $\mathbf{z = x + y}$}}
    \label{fig:ast-pt}
\end{figure}

We then convert the AST to the parse tree. In AST, non-terminals can hold values. For example, in figure~\ref{fig:ast-pt}, node $n_1$ and $n_2$ in the AST hold a values(`$=$' and `$+$') although they are non-terminals. For our model, we only wanted terminals to hold values. Hence, we converted the AST to a parse tree. pulling the value of a non-terminal as a terminal child of that non-terminal in appropriate position. In AST generated by GumTree, Java language constructs (such as `$;$', `$($', `$)$') are also encoded implicitly in the AST. We did not want that either. We searched in the source code for missing tokens and added those in appropriate positions as terminals.

% \subsubsection{Grammar Extraction}
% \label{subsub:grammar}
% We construct a set of production rules from the parse trees we constructed for the dataset. We call it approximate Java parsing Grammar, $\mathscr{G}$. We use this grammar 
\subsection{Tree2Tree Translation Model}
\label{subsec:training}
 One such improvement was also capturing the syntactic information from the syntax tree (tree encoder). Since we are dealing with code and code is highly structured, we adopt the tree-structured encoder. We deploy a bottom-up tree-structured neural network to encode the syntactic information of the source code. 
 \todo{...}
 
Given a source code $x$, our goal is to predict the most imminent change to $x$ and generate a new code snippet $y$.  Our goal is to generate $y$ such that it maximizes $p(y|x)$. To implement such a machine learning model, we turn to NMT-style models.
There are multiple design decisions involved when designing such a machine learning models. Given the well-known structure of code, we depart from standard natural language models and formulate both $x$ and $y$ as parse trees. Once we generate $y$ as a parse tree, we can easily do a tree-walk and convert the tree to code. 


\subsubsection{The Model}
Like every NMT system, the model consists of two main parts, an encoder and a decoder. The encoder takes input $x$ and extracts features that are relevant to the decoder which uses those features to inform the generation process of $y$. 


\textbf{Encoder} For encoding $x$, we adopt similar encoding technique proposed by Chen~\etal~\cite{chen-EtAl:2017:Long6}. The source code $x$, is a sequence of tokens $w_1, w_2, ..., w_n$. At first, we follow the procedure described by Bahdanau~\etal~\cite{bahdanau2014neural} to compute hidden representation for each token. At this stage, for every token, the hidden representation of each token contains information about itself and the tokens that precede and follow it. To compute this, we deploy a bidirectional GRU (biGRU). This contains two Gated Recurrent Unit (GRU), one in forward direction (resulting $h_i^f$, the forward representation of each $w_i$), another in backward direction (resulting $h_i^b$, the forward representation of each $w_i$). Thus the bi-directional representation of token $w_i$ is 
\begin{equation}
\label{eqn:h-bidir}
    h_i = \left[
        \begin{array}{l}
             h_i^f\\
            h_i^b
        \end{array}
        \right]
\end{equation}
So far, this $h_i$ captures the sequential dependencies among the tokens. However, since code is highly structured, we use the syntax structure of $x$. We populate each token (terminal node) of the syntax tree of $x$ with the corresponding $h_i$ generated by equation~\ref{eqn:h-bidir}. Then, we calculate the hidden representation of each node from its children nodes representation recursively. 
For instance, to compute the representation of a node $n$ with children $C = [c_1, c_2, ..., c_k]$, we compute the hidden representation $H_n$ using the following equation,
\begin{equation}
    \label{eqn:h-top}
    H(n) = \begin{cases}
    h_i & \text{if n is a leaf node}\\
    E(C) & \text{if n is non-leaf node}
    \end{cases}
\end{equation}
Where the encoding function $E$ is defined as,
\begin{equation}
    \label{eqn:encode}
    E(C) = \begin{cases}
    H(c_1) & \text{if }|C| = 1\\
    f\left(W_L^e H(c_1) + W_R^e E(c_2, ..., c_k)\right) & otherwise\\
    \end{cases}
\end{equation}
Here, $f(\phi)$ is a non-linear transformation of input $\phi$. $W_L^e$ and $W_R^e$ are two matrices, which are also learned during the training. We calculate the hidden representation of root $H_{root}$ following equation~\ref{eqn:h-top}. 

\textbf{Decoder} At a high level, we follow Yin~\etal's conditional attention decoder for deriving a sequence of actions. Applying those actions sequentially from the root will yield a complete parse tree. In the heart of the decoder, there is a LSTM, that generates hidden state $s_t$. There are four inputs to the decoder LSTM, \ie i. the action at previous time step ($a_{t-1}$), ii. the action at parent node ($a_{p_t}$), iii. the hidden state at parent node ($s_{p_t}$), and iv. current frontier node ($n_f^t$). The decoder LSTM updates the decoder hidden state as follows:
\begin{equation}
    \label{eqn:decode-h-update}
    s_t = f_{LSTM}([a_{t-1},a_{p_t}, s_{p_t}, n_f^t, c_t], s_{t-1})
\end{equation}
On top of the vanilla LSTM, we used soft attention over the source hidden vectors of all node representations in the source tree($\{H(n)\}$s) to compute the context vector $c_t$. We use these $c_t$ and $s_t$ subsequently to compute several probability distributions. 
\begin{multline}
    \label{eqn:rule-prob}
        p(r|x,  a_1...a_{t-1}, n_f^t) = softmax((E_R .\\
        (W_R  s_t + b_R )  mask_r(n_f^t))
\end{multline}
% \end{equation}
Equation~\ref{eqn:rule-prob} gives a probability distribution over all grammar rules at time $t$. $E_R$, $W_R$, and $b_R$ are parameters that are optimized during training, $mask_r(n)$ is a function that provides a Boolean mask for filtering out improbable rules depending on the type of node $n$ (in this case $n_f^t$). This mask function is a property of the programming language grammar $\mathscr{G}$ and can be statically pre-computed.
We then pick an action $a_t$ from $p\left(a_t = ApplyRule(r = \hat{r}) | x,  a_1...a_{t-1}\right)$ by sampling from the discrete probability distribution given by equation~\ref{eqn:rule-prob}.

If the model chose to select InsertToken action, we either select token from the vocabulary or copy token from source. relevant probability distributions are given by, 
\begin{multline}
    \label{eqn:vocab-prob}
    p(v|x, a_1...a_{t-1}, n_f^t) =  softmax((E_V \\
        (W_V  s_t + b_V )  mask_t(n_f^t))
\end{multline}
Like equation~\ref{eqn:rule-prob}, here also $E_V$, $W_V$, and $b_V$ are parameters and will be learned. Note that, not all terminal nodes can generate all tokens. For instance, there are only 2 possible values for terminal node of type Boolean \ie \texttt{true} and \texttt{false}. So letting the model generate other tokens will always lead to incorrect code. Although, in theory, the model could learn this itself, using the $mask_t(n)$ allows us to expedite the process of learning and does \emph{not} spend model capacity for learning a deterministically known fact. This mask is a 0/1 mask over the vocabulary and can be pre-computed.

In contrast to Yin~\etal, that is learning to generate code given natural language as input, we can take advantage of the fact that tokens that appear in $x$ will also appear in $y$. To use this fact, we turn to copying mechanisms, originally proposed by Vinyals~\etal~\cite{vinyals2015pointer}. It is a neural architecture to learn the conditional probability distribution of an output sequence to positions in an input sequence. It uses an attention mechanism as a pointer to select input token to be copied to the output sequence. The conditional probability of an input token being copied to output sequence is given by, 
\begin{equation}
    \label{eqn:ptr-net}
    p(w_i|copy,x,a_1a_2...a_{t-1}) = \frac{exp(\omega(h_i, [s_t, c_t]))}{\sum_{j=1}^{j=n} exp(\omega(h_j, [s_t, c_t]))}
\end{equation}
Here, $\omega(\phi)$ refers to the function of a deep feed-forward neural network with input $\phi$. Equation~\ref{eqn:ptr-net} gives a probability distribution over all tokens(positions) in the input sequence. We use this probability to add to final probability of an output token. 

Since we are dealing with code changes, not all the tokens from the source should be copied. We wanted to let the model generate tokens. We let the model learn another probability that tells us when to copy. The model calculates that probability as equation~\ref{eqn:copy-prob}.
\begin{equation}
    \label{eqn:copy-prob}
    p(copy_t|x, a_1...a_{t-1}) = softmax(W_C s_t)
\end{equation}
% which is the probability of applying copying.
% \sk{describe copying probability
% }as-is (even if $w_t$ has never been seen in training) the token $w_t$ where $\{w1,w2,...,w_n\} \in x$. 


Finally putting the two attention mechanisms together,
\begin{multline}
    p(a_t = InsertToken(v = \hat{v}) | x, a_1...a_{t-1}, n_f^t) \\
            = (1 - p(copy_t|x, a_1...a_{t-1})) *  p(v = \hat{v}|x, a_1...a_{t-1}, n_f^t)\\
            + p(copy_t|x, a_1...a_{t-1}) * p(w = \hat{v}|copy, x, a_1a_2...a_{t-1})
\end{multline}
and the probability distribution for action at time $t$ becomes,
\begin{multline}
    p(a_t | x, a_1...a_{t-1}) = \\
    \begin{cases}
    p(a_t = ApplyRule | x,  a_1...a_{t-1}, n_f^t) & \text{if } n_f^t \text{ is non-leaf}\\
    p(a_t = InsertToken | x, a_1...a_{t-1}, n_f^t) & \text{if } n_f^t \text{ is leaf}
    \end{cases}
\end{multline}


\subsubsection{Training procedure}
To train the model described above, we first sorted the commits in out dataset based on the chronology. The motivation is, developer can train a model based on earlier changes only. Then developer can deploy a trained model subsequent changes. In line with that motivation, we divided our dataset in 2 parts. First 80\% data are kept as training data and latter 20\% are kept as testing data. During training, we keep 5\% of the training data aside to use as validation data. In training, the objective is to optimize the parameters to maximize probability estimation of equation~\ref{eqn:a_t}. We used cross-entropy loss based of this probability estimation as objective function. To optimize the parameters in the model, we used Adam optimizer.  However, in our preliminary experiment, we found that, the quality of generated code is not directly related to the loss. To mitigate this problem, we used BLEU score~\cite{papineni2002bleu} as an alternative way of measuring the performance of trained model. We run the training model for a fixed amount of time ($n_{epoch}$). However, if the model performance (in terms of BLEU score) on validation data does not improve consecutively over a fixed number of steps ($valid_{patience}$), we stop training procedure and declare the best resulting model as the target model. Since throughout all $valid_{patience}$ training iteration, the model could produce better result on validation dataset, our decision for early stop is rational. We believe the model had reached optima.  \sk{once sentence: optimization with Adam(?), hidden size of vectors \etc}

\subsection{Testing and Deployment of the Model}
\label{subsec:testing}
\begin{algorithm}[htb]
    \caption{Beam Search Algorithm for Inferring Changed Code. $x$ is the input code, $\mathscr{G}$ is the Grammar.}

\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Return}{return}
\underline{\textbf{Function beam-search($x$)}} \\
\SetAlgoVlined
\Input{$x$ - input code}
\Output{$[y]$ - list of codes after changes}
 $init\_state = Encoder(x)$\\
 $root\_hyp = Hypothesis(init\_state)$\\
 $all\_hyps = [root\_hyp]$\\
 $completed\_hyps = []$\\
 \For{i = 1 to max\_timestep}{
      $new\_hyps = []$\\
      \For{q in all\_hyps}{
        \eIf{$q.n_f^t\text{ is non-terminal}$}{
            \For{$rule \in \mathscr{G}$}{
                $q' = q.ApplyRule(rule)$\\
                $q'.score = q.score + rule.log\_prob$\\
                add $q'$ to new\_hyps\\
            }
        }{
            \For{$v \in Vocab$}{
                $q' = q.InsertToken(v)$\\
                $q'.score = q.score + v.log\_prob$\\
                \eIf{$q'.isCompleted()$}{
                    add $q'$ to completed\_hyps\\
                }{
                    add $q'$ to new\_hyps\\
                }
            }
        }
      }
      $\text{sort new\_hyps based on score}$\\
      $\text{all\_hyps = top k Hypotheses fron new\_hyps}$\\
  }
 sort completed\_hyps based on score\\
 \Return{top $K$ hypotheses from completed\_hyps}
 \label{alg:inference}
\end{algorithm}
To deploy a model and generate code, we adopt beam-search method. In beam search, instead of greedily generating one $y$, we search for a sorted set of $K$ hypotheses.

At each time step, we pick the top $K$ partial expansions. Then, we explore all states reachable from those $K$ states. If we find a state that is completed (\ie a state containing a complete tree), we exclude that hypothesis from being expanded further. We then pick top $K$ incomplete hypotheses based on the score. We stop this process if max time step is reached or if there is no more incomplete hypothesis to be expanded. We then sort all completed hypotheses based on the score and  generate code from top $K$ hypotheses. The inference procedure is articulated in Algorithm~\ref{alg:inference}. 


==> backups/background_back.tex <==
\section{Background}
\label{sec:background}

% There are multiple design decision involved when designing a machine learning
% models of code. One such decision is how code is represented within the machine learning component.
% Almost always it is impossible to represent source code as a single entity 
% and thus a design decision on how to represent code is needed.
% A large proportion of the literature, resorts in representing source code as a sequence of
% tokens. Such models, although successful in many tasks, capture some of the
% statistical properties of the code, but mostly fail to capture its rigid and
% rich syntactic structure. Syntactic machine learning
% models capture the parse or abstract syntax tree (AST) of the code. These models
% can take advantage of the syntactic structure but may still fail to capture
% some semantic information of the code, such as variable scopes. Finally, graph models
% of code can capture code's rich syntactic and semantic nature to the extend
% that such features can be extracted.

% In this work, we are interested in machine learning models that generate source code
% edits, which is a special case of the very general code generation problem. Code
% synthesis models is one kind of such model but take into account additional
% specification such as input-output examples or formal constraints. Such models
% often rely on formal methods or combinations of formal and machine learning
% methods. In contrast, in this work we are interested in statistical models
% that can predict a piece of code given only a previous version of that code and thus we
% need to turn to statistical methods. 

% Generating source code in machine learning has been explored in the past. The
% generation process for token-based models is straightforward; tokens are
% generated sequentially one after the other. Syntactic models also follow
% a straightforward process, where the left-most, bottom-most non-terminal
% is expanded at each timestep. To our knowledge, no other method of code
% generation has been explored in the literature. In our work, we select
% to use a syntactic model of code generation. We are specifically inspired
% by the syntactic code generation of Yin~\etal~\cite{yin2017syntactic} who
% generate code segments for the NLP problem of semantic parsing. We
% describe our model in detail Section~\ref{subsec:syntacticGeneration}.

% A machine learning-based code generation model represents a probability
% distribution $P(c|\kappa)$ where $c$ is the code being generated and
% $\kappa$ is the contextual information that is used during code generation.
% Language models of code have no context, \ie $\kappa=\varnothing$.
% ~\sk{Baishakhi: one can argue that context of n-gram model is the previous token sequences.}
% Using language models to predict code edits would be
% pointless, since such models cannot use any information about the
% original version of the code.
% Instead, one natural probabilistic model of code edits are
% machine translation-style models, that model $P(c|s)$ where $s$
% is the source input and $t$ the target input. Natural language
% translation is a special case of such a model, where $c$, for example
% is a sentence in English and $s$ a sentence in French. These models
% naturally allow us to model code edits, taking into consideration
% the original code and defining a conditional probability distribution of the target code.
% Such models have been used for source code migration from one programming
% language into another~\cite{karaivanov2014phrase,nguyen2014statistical,chen2018tree}.
% Closer to code edits, such models have also been explored in NLP for paraphrasing~\cite{mallinson2017paraphrasing}. 
% Finally, we note that existing work has considered cases where
% $\kappa$ is information from another modality, such as natural language text~\cite{allamanis2015bimodal,yin2017syntactic}.

\subsection{Syntactic Code Generation}
\label{subsec:syntacticGeneration}
In this work, we are interested in generating some code $y$ in its syntactic form. Such machine learning models have been explored, but not for the code change modeling task~\cite{maddison2014structured,bielik2016phog,yin2017syntactic}. Here, we briefly describe one of the most recent models. At a high level, these models  adopt a top-down, left-to-right tree expansion, where the bottom-most, left-most non-terminal is expanded at each timestep. The derivation process is a sequential application of grammar rules, and generation of terminal tokens. 

In our work, we base our code generation model on the work of Yin~\etal~\cite{yin2017syntactic} who design a text-to-code model for semantic parsing. We briefly explain their code generation model here. We start from a root node. We maintain a pointer to the frontier node. At the beginning ($t = 0$), root is the frontier node.  At each time step of deriving the target parse tree, the frontier node is expanded in one of the following 2 ways.  
\begin{itemize}
    \item \textbf{ApplyRule($r$)}: This action generates the program structure, expanding the frontier node ($n_{f}^t$) in a depth-first, left-to-right fashion. From the fixed set of grammar rules of $\mathscr{G}$, ApplyRule selects a rule to expand $n_{f}^t$ and uses that to grow the tree structure. However, not all the rules can be applied at a particular time instance. To overcome this problem, we only consider the rules whose rule head type is of the type of $n_{f}^t$. We use a Boolean mask to do so and consider from the rules that are plausible to apply. In this way, we guarantee that the resultant tree can be fully generated and will be compilable. 
    % A rule of the format $r -> x ... y$ is applied to the current derivation tree, if the frontier node is a non-terminal. 
    \item \textbf{InsertToken($v$)} : At any time instance, if the frontier node($n_f^t$) is a terminal, this action is applied. This action first select a token probabilistically either from the vocabulary or the source code. After selecting a token($v$), this action puts the $v$ as a value of $n_f^t$. Then it removes $n_f^t$ as frontier node marking that branch of derivation as fully derived and proceeds on to the next frontier node.  
\end{itemize}
Formally, this model can be described by the probability of the derived tree, conditioned on a possibly empty context $c$ to be 
\begin{equation}
\label{eqn:a_t}
    p(y|c) = \prod_{t=1}^{T} p(a_t|c, a_1...a_{t-1})
\end{equation}
where $a_t$ is the action at time step $t$. It is to be noted here that at time step $t$, the probability of $a_t$ is not only dependent on the context ($c$), but also on the previously taken actions $a_1...a_{t-1}$). 

==> backups/background_backup1.tex <==
\section{Background}
\label{sec:background}

Generating source code using machine learning models has been explored in the past~\cite{hindle2012naturalness,Tu:2014:FSE,hellendoorn2017deep,parvez2018building}. Such models can be represented as a probability distribution $P(c|\kappa)$ where $c$ is the code being generated and $\kappa$ is the contextual information upon which the generated code is conditioned upon. 

In this work, as opposed to generating code, we want to generate {\em code edits}, \ie how a piece of code changes. 
Thus, we are interested in a model that can predict a piece of code given its previous version.
This can be achieved using {\em Neural Machine Translation} (NMT), which is a special case of probability distribution $P(c|\kappa)$, where $c$ is the new and $\kappa$ is the previous version of the code. 
The translation model will learn the transformation %(\ie mapping) 
between the two code versions. % (similar to learning the mapping between two languages, \eg English to French). 
Thus, NMT allows to represent code edits using a single end-to-end model, taking into consideration the original version of a code and defining a conditional probability distribution of the target version. 
Such probability distribution can be written as $P(t|s)$, where $s$ and $t$ correspond to the source and target of the edits. 
Similar to code edits, such models have also been explored in NLP for paraphrasing~\cite{mallinson2017paraphrasing}. 

%Finally, we note that existing work has considered cases where $\kappa$ is information from another modality, such as natural language text~\cite{allamanis2015bimodal,yin2017syntactic}.

% In machine translation, there are several methods for translating sentence/phrase from one corpus to another. Since all the languages do not follow the same grammar, the Neural Machine Translation (NMT) model learns the transformation pattern that makes a successful translation. 

NMT models are usually a cascade of an Encoder and a Decoder. The most common and successful NMT model is sequence-to-sequence (seq2seq) model~\cite{bahdanau2014neural}, where the input is treated as a sequence of tokens and encoded by a sequential encoder (\eg an LSTM). The output of the encoder is stored in an intermediate representation.
Next, the decoder decodes the encoder output and 
produces a stream of tokens. In NMT literature, several improvements have been made over the base seq2seq model, such as attention~\cite{bahdanau2014neural} and copying~\cite{allamanis2016convolutional}. Briefly, attention mechanism allows a model to automatically (soft-)search for parts of the source that are important in predicting a target. Copying is a special type of attention mechanism, where, the searched portion of the source is directly copied to the target. We employed both attention and copying mechanisms in this work. 

Although for natural language text, a seq2seq NMT has proved successful, applying NMT to source code we need to consider different design decisions.
One of them is how to represent code within the machine learning component. 
%Almost always it is impossible to represent source code as a single entity, and thus a design decision on how to represent code is needed. 
A large proportion of the literature resorts in representing source code as a sequence of tokens~\cite{ray2016naturalness, Tu:2014:FSE, hindle2012naturalness}. Such models, although successful in many tasks, capture some of the statistical properties of the code, but mostly fail to capture its rigid and rich syntactic structure. Syntactic machine learning models~\cite{parvez2018building, yin2017syntactic} capture the parse or abstract syntax tree (AST) of the code. These models can take advantage of the syntactic structure but may still fail to capture some semantic information of the code, such as variable scopes. Finally, graph models~\cite{nguyen2015graph,allamanis2017learning} of code can capture code's rich syntactic and semantic nature to the extent that such features can be extracted. However, generating code directly as a graph has not been explored.
% Generating source code in machine learning has been explored in the past. The
% generation process for token-based models is straightforward; tokens are
% generated sequentially one after the other. Syntactic models also follow
% a straightforward process, where the left-most, bottom-most non-terminal
% is expanded at each timestep. To our knowledge, no other method of code
% generation has been explored in the literature. 
In our work, we select to use a syntactic model of code generation. Since we are interested in learning the edits from the wild, semantic information was not very relevant to us. Thus, a graph-based model might have been overkill.


%We are specifically inspired by the syntactic code generation of Yin~\etal~\cite{yin2017syntactic} who generate code segments for the NLP problem of semantic parsing.
%We describe our model in detail in~\Cref{sec:approach}.




==> backups/intro-backup.tex <==
%!Tex root=./main.tex

\IEEEraisesectionheading{\section{Introduction}\label{sec:intro}}

Developers often edit source code to add new features, fix bugs, or maintain existing functionality (\eg API updates, refactoring, \etc.). Recent research has shown that these edits are often repetitive~\cite{nguyen2010recurring,nguyen2013study,ray2014uniqueness}. Moreover, the code components (\eg token, sub-trees, \etc.) used to build the edits are often times taken from the existing codebase~\cite{martinez2014fix, barr2014plastic}. However, manually applying such repetitive edits can be tedious and error-prone~\cite{ray2013detecting}. Thus, it is important to automate code changes, as much as possible, to reduce the developers' burden. 

There is a significant amount of industrial and academic work on automating code changes. For example, modern IDEs support specific types of automatic changes (\eg refactoring, adding boiler-plate code~\cite{vstudio,eclipse}, \etc). Many research tools aim to automate some types of edits, \eg API related changes~\cite{nguyen2010graph,tansey2008annotation,raychev2014code,andersen2012semantic,padioleau2008documenting,nguyen2016api}, refactoring~\cite{foster2012witchdoctor,raychev2013refactoring,ge2012reconciling,meng2015does}, \etc.  Researchers have also proposed to automate generic changes by learning either from example edits~\cite{meng2011systematic,rolim2017learning} or from similar patches applied previously to source code~\cite{meng2013lase,nguyen2013study,ray2014uniqueness}.

While the above lines of work are promising and have shown initial success, they either rely on predefined change templates or require domain-specific knowledge: both are hard to generalize in the larger context. However, all of them leverage, in someway, common edit patterns. Given that a large amount of code and its change history is 
available thanks to software forges like GitHub, Bitbucket, \etc., 
a natural question arises: {\em Can we learn to predict general code changes by learning them in the wild?}  

Recently there has been a lot of interest in using machine learning techniques to model and predict source code from real world~\cite{allamanis2018survey}. However,  modeling changes is different from modeling general code generation, since modeling changes is conditioned on the previous version of the code. In this work, we research whether machine learning models can capture the repetitiveness and statistical characteristics of code edits that developers apply daily. Such models can automate code changes, bug fixes, and other software-evolution-related tasks. 


To this end, we use the general framework of Neural Machine Translation (NMT) to learn from past code changes and suggest future edits. In natural language processing (NLP), NMT is widely used to translate text from one language (\eg English) to another (\eg Spanish). NMT seem to be a natural fit for modeling code changes since it can learn the transformation (\ie edits) from an original to a changed version of the code. Essentially, these models learn the probability distribution of changes and assign higher probabilities to plausible code edits and lower probabilities to less plausible ones. 
% In fact, Tufano \etal~\cite{tufano2018nmt_bug_fix, tufano2019learning} show the initial promise of using a sequence-to-sequence translation model (seq2seq) for fixing bugs and predicting code changes.
In fact, Tufano \etal~\cite{tufano2018nmt_bug_fix, tufano2019learning} show an initial promise of using standard sequence-to-sequence translation model (seq2seq) for predicting abstract code changes.

%For evaluation purpose, we collected 44382 patches from 54 different open project source code repositories. Our experiments show \tool can achieve 26.53\% accuracy in top 20 while recommending abstract patches and  6.33\% accuracy in top 20 while recommending concrete patch which is 96.96\% and 42.25\% higher than \sts bases models. We evaluated \tool performance in recommending bug-fix patches in Defects4j dataset. \tool can produce 8 complete fixes and 2 partial fixes out of 80 bugs in Defects4j dataset.

In this work, our goal is to predict concrete code changes. 
To do that, we design an encoder-decoder-based NMT model that works in two steps. 
First, it learns and suggests structural changes in code using a tree-based translation model. 
Structural changes are suggested in the form of Abstract Syntax Tree (AST) modifications. 
Tree-based models, unlike their token-based counterparts, capture the rich structure of code and produce syntactically correct patches.
Then, we concretize each code fragment generating the tokens conditioned on the AST generated in the first step. Here, given the type of each leaf node in the syntax tree, our model recommends concrete tokens of the correct type while respecting scope information. We combine these two models to realize \tool, a code change suggestion engine, which takes a code fragment as input and generates potential edits of that snippet. 
 
Synthesizing patches (or code in general) is a tough problem~\cite{flener2012logic}. When we view code generation as a sequence of token generation problem, the space of the possible actions becomes too large. Existing statistical language modeling techniques (\eg Raychev~\etal~\cite{raychev2014code}, Tu~\etal~\cite{Tu:2014:FSE}) endorse the action space with a probability distribution, which effectively reduces the action space significantly since it allows to consider only the subset of probable actions. The action space can be further reduced by relaxing the problem of concrete code generation to some form of abstract code generation, \eg generating code sketches~\cite{murali2017neural}, abstracting token names~\cite{tufano2018nmt_bug_fix}, \etc. 
For example, Tufano~\etal reduce the effective size of the action space to $3.53 \cdot 10^{10}$ by considering abstract token names~\cite{tufano2018nmt_bug_fix}. 
While considering all possible ASTs allowed by the language's grammar, the space size grows to $1.81\cdot 10^{35}$.
In this work, a probabilistic grammar further reduces the effective action space to $3.18\cdot 10^{10}$, which is significantly lower than previous methods.
Thus, the reduction of the action space allow us to search for code more efficiently.



% We design an encoder-decoder-based machine translation model that operates on the tree representation of the code to capture syntactic changes. Our key observation is that such tree-based models, unlike their token-based counterparts, can capture the rich structural properties of code and thus can produce syntactically correct patch. 
% In particular, we deconstruct the change suggestion in two steps. First, we learn and suggest structural changes in code using a tree-based translation model. This step suggests potential structural changes that can be applied to the   Abstract Syntax Tree (AST) of a code fragment. Next, we generate concrete code fragment conditioned on the AST generated in the first step. Here, given an AST type, we try to recommend a concrete token of that type which is also in the scope. We combine these two models to realize a code change suggestion engine, \tool, which takes an unmodified code fragment as input and suggests potential changes. 

% We deconstruct the code change suggestion in two steps. Our first step is to learn and suggest structural changes in a code. We realize this task with tree-based translation model. The goal of this model is to suggest structural changes (if any) in a given AST of the code. The second and the last step is to generate code conditioned on the AST generated in the first step. While generating every token for the code, since we already know the AST type for each token (from step 1), the search space is significantly reduced.  
% We combine these two models to realize a code change suggestion engine, \tool, which takes an unmodified code fragment as input and suggests potential changes. 

% \rayb{Please read this paragraph.}
% Synthesizing the changed code is an integral part of code change generation problem. Synthesizing a patch (or code in general) is a tough problems~\cite{flener2012logic}. When we view code generation as sequence of token generation problem, the space of the possible actions is too large. However, statistical language modeling techniques (such as approaches proposed by Raychev~\etal~\cite{raychev2014code}, Tu~\etal~\cite{Tu:2014:FSE}) endorse the action space with a probability distribution. When only the probable actions are considered the action space becomes significantly smaller. The action space can be further reduced by relaxing the problem of code synthesis. For instance, Murali~\etal~\cite{murali2017neural} propose to use code sketches,  Tufano~\etal~\cite{tufano2018nmt_bug_fix} propose using abstract names to reduce the action space. 
% In this work, we are proposing to use the programming language grammar. Our approach of generating ASTs which are then concretized can be viewed as a high-level generalization of Sketch-based code synthesis~\cite{murali2017neural}. While the sketch-based approach deals with generating code from problem description and/or auxiliary information, we tackle a different problem of learning and applying probable code change patterns. 
% Step 1 of \tool is also generating code template. However, to extract rich syntactic structure of the code, we leverage Abstract Syntax Tree of the code as template. In contrast to Tufano~\etal~\cite{tufano2018nmt_bug_fix}'s search over abstract token space, we search over rules from Context Free Grammar(CFG) space. We further transformed the CFG into  Probabilistic CFG (PCFG) to reduce the search space even more. Our analysis shows that, average size of search space reduces quite significantly while we transform CFG to PCFG. And the size of PCFG search space is significantly lower than the that of abstract token's. 

% Synthesizing the changed code is an integral part of code change generation problem. Synthesizing a patch (or code in general) is a tough problems~\cite{flener2012logic}. When we view code generation as sequence of token generation problem, the space of the possible actions is too large. However, statistical language modeling techniques (such as approaches proposed by Raychev~\etal~\cite{raychev2014code}, Tu~\etal~\cite{Tu:2014:FSE}) endorse the action space with a probability distribution. When only the probable actions are considered the action space becomes significantly smaller. The action space can be further reduced by relaxing the problem of code synthesis. For instance, Murali~\etal~\cite{murali2017neural} propose to use code sketches,  Tufano~\etal~\cite{tufano2018nmt_bug_fix} propose using abstract names to reduce the action space. 
% In this work, we are proposing to use the programming language grammar. Our approach of generating ASTs which are then concretized can be viewed as a high-level generalization of Sketch-based code synthesis~\cite{murali2017neural}. While the sketch-based approach deals with generating code from problem description and/or auxiliary information, we tackle a different problem of learning and applying probable code change patterns. 
% Our analysis shows the average size of action space is $3.53*10^{10}$ when we abstract token names by symbolic names. The action space is $1.81*10^{35}$, if we generate ASTs using context-free grammar (CFG) production rules from a context-free language. However, when we convert the CFG to a Probabilistic CFG, the effective size of the action space goes down to $3.18*10^{10}$, which is significantly lower than that of CFG-based and symbolic names-based action space. 

In this work, we collect a new dataset~\textemdash~\dataname, consisting of 44372 patches from 48 open-source GitHub projects collected from Travis Torrent~\cite{msr17challenge}. Our experiments show \tool achieves 15.81\% patch suggestion accuracy in the top 10 suggestions; this result outperforms a \sts based model by 98.16\%. \tool can also predict 33.61\% of structural changes accurately within the top 10 suggestion. We also evaluate \tool on \icsedata proposed by Tufano~\etal~\cite{tufano2019learning}. Our evaluation shows that \tool suggests 14.36\% of correct patches in the top 10 outperforming \sts-based model by 108.2\%. 
Furthermore, we leveraged \tool's ability to learn bug fix patterns from \onelinetrain dataset. \tool can generate 27 patches from 75 one line bugs in \defj dataset. Among these 27 patches, 20 are semantically identical to the patches developer provided. 
% Further evaluation on \tool's ability to suggest bug-fixing patches in \defj shows that \tool suggests 16 complete fixes and 9 partial fixes out of 80 bugs in \defj. 
%
% these patches are similar to change templates suggested by modern IDEs. \tool can also suggest concrete patches with 6.33\% accuracy in the top 20. These results are 96.96\% and 42.25\% better than a \seq based model, which is the most common way to model natural language translation. 
% We further evaluate \tool's performance in suggesting bug-fix patches of Defects4J dataset. \tool can produce 8 complete fixes (\ie 10\%) and 2 partial fixes out of 80 bugs in the Defects4J dataset.
%
%
In summary, our key contributions are: 
% \vspace{-3pt}
\begin{itemize}[leftmargin=*,label=-]
    \item 
We propose a novel tree-based code editing machine learning model that leverages the rich syntactic structure of code and generates syntactically correct patches. To our knowledge, we are the first to model code changes with tree-based machine translation.
\item 
We collect a large dataset of 44k real code changes.
\item 
We implement our approach, \tool, and exhaustively evaluate the viability of using \tool for suggesting patch templates, concrete changes, and bug fixes. 
\end{itemize}
We will release our code and data for broader dissemination. 

==> backups/intro_bck.tex <==
%!Tex root=./main.tex

\IEEEraisesectionheading{\section{Introduction}\label{sec:intro}}

Developers often edit source code to add new features, fix bugs, or maintain existing functionality (\eg API updates, refactoring, \etc.). Recent research has shown that these edits are often repetitive~\cite{nguyen2010recurring,nguyen2013study,ray2014uniqueness}. Moreover, the code components (\eg token, sub-trees, \etc.) used to build the edits are often times taken from the existing codebase~\cite{martinez2014fix, barr2014plastic}. However, manually applying such repetitive edits can be tedious and error-prone~\cite{ray2013detecting}. Thus, it is important to automate code changes, as much as possible, to reduce the developers' burden. 

There is a significant amount of industrial and academic work on automating code changes. For example, modern IDEs support specific types of automatic changes (\eg refactoring, adding boiler-plate code~\cite{vstudio,eclipse}, \etc). Many research tools aim to automate some types of edits, \eg API related changes~\cite{nguyen2010graph,tansey2008annotation,raychev2014code,andersen2012semantic,padioleau2008documenting,nguyen2016api}, refactoring~\cite{foster2012witchdoctor,raychev2013refactoring,ge2012reconciling,meng2015does}, \etc.  Researchers have also proposed to automate generic changes by learning either from example edits~\cite{meng2011systematic,rolim2017learning} or from similar patches applied previously to source code~\cite{meng2013lase,nguyen2013study,ray2014uniqueness}.

While the above lines of work are promising and have shown initial success, they either rely on predefined change templates or require domain-specific knowledge: both are hard to generalize in the larger context. However, all of them leverage, in someway, common edit patterns. Given that a large amount of code and its change history is 
available thanks to software forges like GitHub, Bitbucket, \etc., 
a natural question arises: {\em Can we learn to predict general code changes by learning them in the wild?}  

Recently there has been a lot of interest in using machine learning techniques to model and predict source code from real world~\cite{allamanis2018survey}. However,  modeling changes is different from modeling generic code generation, since modeling changes is conditioned on the previous version of the code. In this work, we research whether machine learning models can capture the repetitiveness and statistical characteristics of code edits that developers apply daily. Such models should be able to automate code edits including feature changes, bug fixes, and other software-evolution-related tasks. 






% To this end, we use the general framework of Neural Machine Translation (NMT) to learn from past code changes and suggest future edits. In natural language processing (NLP), NMT is widely used to translate text from one language (\eg English) to another (\eg Spanish). NMT seem to be a natural fit for modeling code changes since it can learn the transformation (\ie edits) from an original to a changed version of the code. Essentially, these models learn the probability distribution of changes and assign higher probabilities to plausible code edits and lower probabilities to less plausible ones. 
% % In fact, Tufano \etal~\cite{tufano2018nmt_bug_fix, tufano2019learning} show the initial promise of using a sequence-to-sequence translation model (seq2seq) for fixing bugs and predicting code changes.
% In fact, Tufano \etal~\cite{tufano2018nmt_bug_fix, tufano2019learning} show an initial promise of using standard sequence-to-sequence translation model (seq2seq) for predicting abstract code changes.

% To this end, we propose a generic model for learning the probability distribution of code changes and automate the process of code change. We implement the proof of concept through an Encoder-Decoder based system. In this system, we first encode a given code fragment to a latent vector representation and then synthesize the target (\ie, changed) code starting with the encoded representation. 
% In this way, we implicitly model and learn the conditional probability distribution of a changed code given the code before the change. Thus, we aim to model %and learn 
% the probability distribution of the code change patterns\textemdash these models learn the probability distribution of changes and assign higher probabilities to plausible code edits and lower probabilities to less plausible ones. In fact, there are several works in literature~\cite{tufano2019learning, tufano2018nmt_bug_fix, chen2018sequencer} which show use of Neural Machine Translation model to model code changes. In this work, we leveraged the building block of any programming language \ie, the Context Free Grammar. We designed a custom probabilistic model that is tailored to work with programming languages.
% Tufano \etal~\cite{tufano2018nmt_bug_fix, tufano2019learning} show an initial promise of using standard sequence-to-sequence translation model (seq2seq) for predicting abstract code changes.

% use the general framework of Neural Machine Translation (NMT) to learn from past code changes and suggest future edits. In natural language processing (NLP), NMT is widely used to translate text from one language (\eg English) to another (\eg Spanish). NMT seem to be a natural fit for modeling code changes since it can learn the transformation (\ie edits) from an original to a changed version of the code. 

% % In fact, Tufano \etal~\cite{tufano2018nmt_bug_fix, tufano2019learning} show the initial promise of using a sequence-to-sequence translation model (seq2seq) for fixing bugs and predicting code changes.


%For evaluation purpose, we collected 44382 patches from 54 different open project source code repositories. Our experiments show \tool can achieve 26.53\% accuracy in top 20 while recommending abstract patches and  6.33\% accuracy in top 20 while recommending concrete patch which is 96.96\% and 42.25\% higher than \sts bases models. We evaluated \tool performance in recommending bug-fix patches in Defects4j dataset. \tool can produce 8 complete fixes and 2 partial fixes out of 80 bugs in Defects4j dataset.

% To this end, we propose a neural model for learning the probability distribution of code changes. Similar to  and leverage the model to automate code change. We implement the proof of concept with an Encoder-Decoder based system, where we first encode a given code fragment to a latent vector representation and then synthesize the target (\ie, changed) code starting with the encoded representation. 
% In this way, we implicitly model and learn the conditional probability distribution of a changed code given the code before the change. Thus, we aim to model the probability distribution of the code change patterns\textemdash these models learn the probability distribution of changes and assign higher probabilities to plausible code edits and lower probabilities to less plausible ones. 

A {\em code edit} can be represented as a tuple of two code versions:$< ${\em prev},{\em target}$ >$. We aim to learn the conditional probability distribution of {\em target} code version given its {\em prev} code version such that a good model will assign higher probabilities to plausible target  version and lower probabilities to less plausible ones.  We realize this with an Encoder-Decoder based system, where prev code version is encoded to a latent vector representation and then the target version is synthesized from the encoded representation. 



In particular, we use encoder-decoder based Neural Machine Translation model similar to previous works~\cite{tufano2019learning, tufano2018nmt_bug_fix, chen2018sequencer}. However, unlike our predecessors who used sequence-to-sequence model to primarily capture changes in token sequences, we design a two step Neural Machine Translation model that jointly models the probability distribution of changes.
First, it learns and suggests structural changes in code using a tree-based translation model. 
Structural changes are suggested in the form of Abstract Syntax Tree (AST) modifications. 
Tree-based models, unlike their token-based counterparts, capture the rich structure of code and produce syntactically correct patches.
Then, we concretize each code fragment generating the tokens conditioned on the AST generated in the first step. Here, given the type of each leaf node in the syntax tree, our model recommends concrete tokens of the correct type while respecting scope information. We combine these two models to realize \tool, a code change suggestion engine, which takes a code fragment as input and generates potential edits of that snippet. 


Some previous works~\cite{tufano2019learning, tufano2018nmt_bug_fix, chen2018sequencer} use sequence-to-sequence Neural Machine Translation model to learn  such changes. Such a sequence-to-sequence model only captures the changes in token sequences.  
%However, changes often modify code structure and semantics. 
%Context-Free-Grammar (CFG) of a programming language can capture the valid code components, as thus valid changes, of a program. 
%To capture such structural changes, we leverage Context-Free-Grammar of the language and design a custom probabilistic model to model code changes.
%In this work, our goal is to predict concrete code changes. 
In contrast, we design a two step Neural Machine Translation model that jointly models the probability distribution of changes.
First, it learns and suggests structural changes in code using a tree-based translation model. 
Structural changes are suggested in the form of Abstract Syntax Tree (AST) modifications. 
Tree-based models, unlike their token-based counterparts, capture the rich structure of code and produce syntactically correct patches.
Then, we concretize each code fragment generating the tokens conditioned on the AST generated in the first step. Here, given the type of each leaf node in the syntax tree, our model recommends concrete tokens of the correct type while respecting scope information. We combine these two models to realize \tool, a code change suggestion engine, which takes a code fragment as input and generates potential edits of that snippet. 
 
Synthesizing patches (or code in general) is a tough problem~\cite{flener2012logic}. When we view code generation as a sequence of token generation problem, the space of the possible actions becomes too large. Existing statistical language modeling techniques (\eg Raychev~\etal~\cite{raychev2014code}, Tu~\etal~\cite{Tu:2014:FSE}) endorse the action space with a probability distribution, which effectively reduces the action space significantly since it allows to consider only the subset of probable actions. The action space can be further reduced by relaxing the problem of concrete code generation to some form of abstract code generation, \eg generating code sketches~\cite{murali2017neural}, abstracting token names~\cite{tufano2018nmt_bug_fix}, \etc. 
For example, Tufano~\etal reduce the effective size of the action space to $3.53 \cdot 10^{10}$ by considering abstract token names~\cite{tufano2018nmt_bug_fix}. 
While considering all possible ASTs allowed by the language's grammar, the space size grows to $1.81\cdot 10^{35}$.
In this work, a probabilistic grammar further reduces the effective action space to $3.18\cdot 10^{10}$, which is significantly lower than previous methods.
Thus, the reduction of the action space allow us to search for code more efficiently.



% We design an encoder-decoder-based machine translation model that operates on the tree representation of the code to capture syntactic changes. Our key observation is that such tree-based models, unlike their token-based counterparts, can capture the rich structural properties of code and thus can produce syntactically correct patch. 
% In particular, we deconstruct the change suggestion in two steps. First, we learn and suggest structural changes in code using a tree-based translation model. This step suggests potential structural changes that can be applied to the   Abstract Syntax Tree (AST) of a code fragment. Next, we generate concrete code fragment conditioned on the AST generated in the first step. Here, given an AST type, we try to recommend a concrete token of that type which is also in the scope. We combine these two models to realize a code change suggestion engine, \tool, which takes an unmodified code fragment as input and suggests potential changes. 

% We deconstruct the code change suggestion in two steps. Our first step is to learn and suggest structural changes in a code. We realize this task with tree-based translation model. The goal of this model is to suggest structural changes (if any) in a given AST of the code. The second and the last step is to generate code conditioned on the AST generated in the first step. While generating every token for the code, since we already know the AST type for each token (from step 1), the search space is significantly reduced.  
% We combine these two models to realize a code change suggestion engine, \tool, which takes an unmodified code fragment as input and suggests potential changes. 

% \rayb{Please read this paragraph.}
% Synthesizing the changed code is an integral part of code change generation problem. Synthesizing a patch (or code in general) is a tough problems~\cite{flener2012logic}. When we view code generation as sequence of token generation problem, the space of the possible actions is too large. However, statistical language modeling techniques (such as approaches proposed by Raychev~\etal~\cite{raychev2014code}, Tu~\etal~\cite{Tu:2014:FSE}) endorse the action space with a probability distribution. When only the probable actions are considered the action space becomes significantly smaller. The action space can be further reduced by relaxing the problem of code synthesis. For instance, Murali~\etal~\cite{murali2017neural} propose to use code sketches,  Tufano~\etal~\cite{tufano2018nmt_bug_fix} propose using abstract names to reduce the action space. 
% In this work, we are proposing to use the programming language grammar. Our approach of generating ASTs which are then concretized can be viewed as a high-level generalization of Sketch-based code synthesis~\cite{murali2017neural}. While the sketch-based approach deals with generating code from problem description and/or auxiliary information, we tackle a different problem of learning and applying probable code change patterns. 
% Step 1 of \tool is also generating code template. However, to extract rich syntactic structure of the code, we leverage Abstract Syntax Tree of the code as template. In contrast to Tufano~\etal~\cite{tufano2018nmt_bug_fix}'s search over abstract token space, we search over rules from Context Free Grammar(CFG) space. We further transformed the CFG into  Probabilistic CFG (PCFG) to reduce the search space even more. Our analysis shows that, average size of search space reduces quite significantly while we transform CFG to PCFG. And the size of PCFG search space is significantly lower than the that of abstract token's. 

% Synthesizing the changed code is an integral part of code change generation problem. Synthesizing a patch (or code in general) is a tough problems~\cite{flener2012logic}. When we view code generation as sequence of token generation problem, the space of the possible actions is too large. However, statistical language modeling techniques (such as approaches proposed by Raychev~\etal~\cite{raychev2014code}, Tu~\etal~\cite{Tu:2014:FSE}) endorse the action space with a probability distribution. When only the probable actions are considered the action space becomes significantly smaller. The action space can be further reduced by relaxing the problem of code synthesis. For instance, Murali~\etal~\cite{murali2017neural} propose to use code sketches,  Tufano~\etal~\cite{tufano2018nmt_bug_fix} propose using abstract names to reduce the action space. 
% In this work, we are proposing to use the programming language grammar. Our approach of generating ASTs which are then concretized can be viewed as a high-level generalization of Sketch-based code synthesis~\cite{murali2017neural}. While the sketch-based approach deals with generating code from problem description and/or auxiliary information, we tackle a different problem of learning and applying probable code change patterns. 
% Our analysis shows the average size of action space is $3.53*10^{10}$ when we abstract token names by symbolic names. The action space is $1.81*10^{35}$, if we generate ASTs using context-free grammar (CFG) production rules from a context-free language. However, when we convert the CFG to a Probabilistic CFG, the effective size of the action space goes down to $3.18*10^{10}$, which is significantly lower than that of CFG-based and symbolic names-based action space. 

In this work, we collect a new dataset~\textemdash~\dataname, consisting of 44372 patches from 48 open-source GitHub projects collected from Travis Torrent~\cite{msr17challenge}. Our experiments show \tool achieves 15.81\% patch suggestion accuracy in the top 10 suggestions; this result outperforms a \sts based model by 98.16\%. \tool can also predict 33.61\% of structural changes accurately within the top 10 suggestion. We also evaluate \tool on \icsedata proposed by Tufano~\etal~\cite{tufano2019learning}. Our evaluation shows that \tool suggests 14.36\% of correct patches in the top 10 outperforming \sts-based model by 108.2\%. 
Furthermore, we leveraged \tool's ability to learn bug fix patterns from \onelinetrain dataset. \tool can generate 27 patches from 75 one line bugs in \defj dataset. Among these 27 patches, 20 are semantically identical to the patches developer provided. 
% Further evaluation on \tool's ability to suggest bug-fixing patches in \defj shows that \tool suggests 16 complete fixes and 9 partial fixes out of 80 bugs in \defj. 
%
% these patches are similar to change templates suggested by modern IDEs. \tool can also suggest concrete patches with 6.33\% accuracy in the top 20. These results are 96.96\% and 42.25\% better than a \seq based model, which is the most common way to model natural language translation. 
% We further evaluate \tool's performance in suggesting bug-fix patches of Defects4J dataset. \tool can produce 8 complete fixes (\ie 10\%) and 2 partial fixes out of 80 bugs in the Defects4J dataset.
%
%
In summary, our key contributions are: 
% \vspace{-3pt}
\begin{itemize}[leftmargin=*,label=-]
    \item 
We propose a novel tree-based code editing machine learning model that leverages the rich syntactic structure of code and generates syntactically correct patches. To our knowledge, we are the first to model code changes with tree-based machine translation.
\item 
We collect a large dataset of 44k real code changes.
\item 
We implement our approach, \tool, and exhaustively evaluate the viability of using \tool for suggesting patch templates, concrete changes, and bug fixes. 
\end{itemize}
We will release our code and data for broader dissemination. 

==> backups/model.tex <==
%!Tex root=./main.tex
%\subsection*{Phase-II.~Tree2Tree Translation Model}
%\label{subsec:training}

\section{Tree2Tree Neural Translation Model}
\label{sec:model}

Our tree2tree NMT model consists of two main parts: an encoder and a decoder. 
% The encoder encodes an input tree $S$ to an intermediate representation, $s'$. 
% The decoder then decodes $s'$ to the target tree $T$.
In this section, we will discuss each of these steps in details.

\subsection{Encoder}
\label{sec:encoder}

For encoding the source tree \told, we adopt a Tree-based GRU model originally developed to translate text from English to Chinese~\cite{chen-EtAl:2017:Long6}. 
It follows two different schemes to encode the terminal and non-terminal nodes. 


\subsubsection{Encoding Terminal Nodes}
The terminal nodes of \told
form a token sequence, say $w_1, w_2, ..., w_n$. For example, in~\Cref{fig:motiv_ed}, the token sequences for the source tree are ({\tt obj,.,val,=,v}). At first, similar to Bahdanau~\etal~\cite{bahdanau2014neural}, for each token, we compute the hidden vector representation that contains information about itself and the tokens that precede and follow it. 
To compute this, we deploy a bidirectional GRU (biGRU)~\cite{chung2014empirical} that employs two Gated Recurrent Unit (GRU), one in forward direction ($f$) and  another in backward direction ($b$). 
The biGRU computes a distributed vector representation of token $w_i$ such that: $\scriptstyle h_i = \left[h_i^f,h_i^b\right]$
where, $h_i$ is the concatenation of the vectors computed by the forward and backward GRUs and represents the token-level information of the terminal nodes of the tree \told. 

\subsubsection{Encoding Non-Terminal Nodes}
For each non-terminal node, we compute the hidden representation from its children nodes' representations recursively using a TreeGRU~\cite{eriguchi2016tree} (\Cref{eqn:h-top}) until the root node is reached. 
For instance, to compute the representation of a node $n$ with children $C = [c_1, c_2, ..., c_k]$, we compute the hidden representation $H(n)$ using the following equation:

\small
\begin{equation}
\label{eqn:h-top}
    H(n) = \begin{cases}
    h_i & \text{if n is a terminal node}\\
    E(C) & \text{if n is non-terminal node}
    \end{cases}
\end{equation}
Where the encoding function $E$ is defined as:
\normalsize
\small
\begin{equation}
    \label{eqn:encode}
    \scriptstyle
    E(C) = \begin{cases}
    H(c_1) & \text{if }|C| = 1\\
    f\left(W_L^e \cdot H(c_1) + W_R^e \cdot E(c_2, ..., c_k)\right) & , otherwise\\
    \end{cases}
\end{equation}
\normalsize
Here, $f(.)$ is a non-linear activation function. 
We used {\tt tanh} in our implementation. 
$W_L^e$ and $W_R^e$ are two matrices, which are also learned during the training. 
We calculate the hidden representation of root $H_{root}$ following ~\Cref{eqn:h-top} ($H_6$ in~\Cref{fig:motiv_ed}), which essentially encodes the whole source tree. 

% \medskip
% \noindent
\subsection{Decoder} 
\label{susec:decoder}

From the intermediate representation, say $s'$, produced by the encoder, the decoder generates the target tree ($T$). 
For a non-terminal node, it generates a subtree, and for a terminal node, it generates its value. 
The tree generation is guided by Java grammar rules whose probability we learn from the training process. At each step of the tree generation, we probabilistically apply these rules.  


\subsubsection{Applying Grammar Rules}
We adopt Yin~\etal's~\cite{yin2017syntactic} probabilistic grammar model 
that represents the tree generation process as a sequence of two types actions: {\tt ApplyRule} and {\tt InsertToken}. 
While the former defines how a tree structure is generated, 
the later defines how the terminal nodes are populated with token values. 

At a given step $t$ during the tree generation process, we expand the bottom-most and left-most node of the current tree. We call such node as {\tt frontier node} ($n_f^t$). 
The tree generation starts from the root node (see~\Cref{fig:motiv_ed}).
%We maintain a pointer to the frontier node. 
Thus, at the beginning ($t = 0$), $root$ is the frontier node. 
We maintain a pointer to the frontier node which updates at every step.
At each time step, the frontier node is expanded using one of the following $actions$:

\noindent
(i) \textbf{ApplyRule($r$)}: 
     This action generates the tree structure by expanding the frontier node ($n_{f}^t$) in a depth-first, left-to-right fashion. From the fixed set of Java grammar rules $\mathscr{G}$, ApplyRule selects a rule $r$ to expand $n_{f}^t$. % to grow the tree structure. 
     In~\Cref{fig:motiv_ed}, $r0$,$r1$,$r2$, $r7$, and $r8$ show these rules.

\noindent     
(ii) \textbf{InsertToken($v$)}: 
At any time instance $t$, if the frontier node($n_f^t$) is a terminal, this action is applied. It selects a token ($v$), probabilistically, either from the vocabulary or the source code and puts $v$ as a value of $n_f^t$. Then it removes $n_f^t$ as frontier node marking that branch of derivation as fully derived and proceeds on to the next frontier node.  
    
% \begin{itemize}[leftmargin=*]
%     \item 
%     \textbf{ApplyRule($r$)}: 
%      This action generates the tree structure, expanding the frontier node ($n_{f}^t$) in a depth-first, left-to-right fashion. From the fixed set of grammar rules $\mathscr{G}$, ApplyRule selects a rule to expand $n_{f}^t$ and uses that to grow the tree structure. In~\Cref{fig:motiv_ed}, $r0$,$r1$,$r2$, $r7$, and $r8$ show these rules.
%      %However, not all the rules can be applied at a particular time instance. To overcome this problem, we only consider the rules whose rule head type is of the type of $n_{f}^t$. 
%     %We use a Boolean mask to do so and consider from the rules that are plausible to apply. 
%     %Here, we use boolean mask to filter out the rules.
%     %Thus, we guarantee that the resultant tree can be fully generated following Java grammar and hence, compilable. 
%     % A rule of the format $r -> x ... y$ is applied to the current derivation tree, if the frontier node is a non-terminal. 
%     \item 
%     \textbf{InsertToken($v$)}: At any time instance, if the frontier node($n_f^t$) is a terminal, this action is applied. It first selects a token 
%     probabilistically either from the vocabulary or the source code. After selecting a token($v$), this action puts the $v$ as a value of $n_f^t$. 
%     Then it removes $n_f^t$ as frontier node marking that branch of derivation as fully derived and proceeds on to the next frontier node.  
% \end{itemize}

Applying these rules sequentially from the root will yield a complete parse tree. In~\Cref{fig:motiv_ed}, rules $r0$ to $r13$ are sequentially applied to generate the final tree. At each step, the rules are selected probabilistically.




%We fed the encoded representation of $AST_{old}$ as $x$.  

\subsubsection{Decoding Scheme}
\begin{figure}[!htpb]
    \centering
    \includegraphics[width=0.9\textwidth]{images/Detailed_step.pdf}

\caption{\small{\textbf{Detailed view of Decoding Scheme at step $\mathbf{t_7}$ (corr.~to rule $\mathbf{r7}$) from~\Cref{fig:motiv_ed}}. 
Here, frontier node (${n_f^t}$) is \texttt{rhs}, parent node is ${stmt}$ at $t_0$. To generate hidden state ${s'_7}$, actions at ${a_0}$ and hidden representation at ${t_0}$~\ie~${s'_0}$ are also fed to the decoder. 
Also, previous action ${a_6}$, context vector ${c_7}$, and frontier node ${n_f^7}$  are fed to the decoder. 
${s'_7}$ is used to compute token and rule probabilities.
\vspace{-2pt}}} 
    \label{fig:detailed_step}
\end{figure}
% \vspace{-30pt}
A decoder generates a target tree (T) given a source context ($S$).
The probability of the final tree, conditioned on a context $S$ is:

\small
\begin{equation}
\label{eqn:a_t}
    p(T|S) = \prod_{t=1}^{\tau} p(a_t|S, a_1...a_{t-1})
\end{equation}
\normalsize

where $a_t$ is the action at time step $t$. 
At any time step $t$, the probability of $a_t$ is not only dependent on the context ($S$), but also on the previously taken actions $a_1...a_{t-1}.$ 
Note that, the source context $S$ generates an intermediate representation $s'$ (encoder's output), which is actually taken by the decoder as input. % that is output by the encoder model (see~\Cref{eqn:h-top}). 
$P$ is calculated by the decoder as explained below. All the intermediate computations are summarized in~\Cref{tab:eq}.

The core of the decoder is an LSTM that generates hidden state $s'_t$ at step $t$. There are five inputs to the decoder LSTM:
(i) the action at previous time step ($a_{t-1}$), 
(ii) the action at parent node ($a_{p_t}$), 
(iii) the hidden state at parent node ($s'_{p_t}$), 
(iv) current frontier node ($n_f^t$), and 
(v) a context vector generated by attention mechanism ($c_t$).~\Cref{fig:detailed_step} shows this step in details. 

% \begin{enumerate}[label=\roman*.]
%     \item The action at previous time step ($a_{t-1}$).
%     \item The action at parent node ($a_{p_t}$), 
%     \item The hidden state at parent node ($s'_{p_t}$), and
%     \item Current frontier node ($n_f^t$). 
%     \item A context vector generated by attention mechanism ($c_t$). 
% \end{enumerate}

At each step $t$, the decoder updates its hidden state using LSTM~\Cref{eqn:decode-h-update} (see~\Cref{tab:eq}).
On top of a vanilla LSTM, we use soft attention over the source hidden vectors of all node representations %in the source tree 
($\{H(n)\}$) to compute the context vector $c_t$. 
We use the hidden state ($s'_t$) subsequently to compute several probability distributions, as shown~\Cref{tab:eq}. 

\input{tables/equation.tex}

Next, the decoder checks the type of the frontier node. If it is a non-terminal node, it applies rules to expand the tree. Otherwise, a token value is selected.

\subsubsection*{Applying Grammar Rules}

At each step of the tree generation, we probabilistically apply the grammar rules.
Equation~\ref{eqn:rule-prob} in~\Cref{tab:eq} gives a probability distribution over all grammar rules at time $t$. 
%$E_R$, $W_R$, and $b_R$ are parameters that are optimized during training, 
$mask_r(n)$ is a function that provides a Boolean mask for filtering out disallowed rules depending on the type of node $n_f^t$. 
This mask function is a property of the Java Grammar $\mathscr{G}$ 
and can be statically pre-computed. We then pick an action $a_t$ from $p\left(a_t = ApplyRule(r = \hat{r}) | S,  a_1...a_{t-1}\right)$ by sampling from the discrete probability distribution given by equation~\ref{eqn:rule-prob}. If the model chose to select InsertToken action, we either select token from the vocabulary or copy token from source $S$. Relevant probability distributions are given by~\Cref{eqn:vocab-prob} 
in~\Cref{tab:eq}.

% \begin{equation}
%     \label{eqn:vocab-prob}
%     \scriptstyle
%     p(v|S, a_1...a_{t-1}, n_f^t) =  softmax((E_V.(W_V s'_t + b_V)mask_t(n_f^t))
% \end{equation}

% \begin{multline}
%     \label{eqn:vocab-prob}
%     \scriptstyle
%     p(v|x, a_1...a_{t-1}, n_f^t) =  softmax((E_V \\
%         (W_V  s_t + b_V )  mask_t(n_f^t))
% \end{multline}

% Like equation~\ref{eqn:rule-prob}, here also $E_V$, $W_V$, and $b_V$ are parameters and will be learned. 

%Note that, not all terminal nodes can generate all tokens.
%For instance, there are only 2 possible values for terminal node of type Boolean \ie \texttt{true} and \texttt{false}. 
%So letting the model generate other tokens will always lead to incorrect code. 
% Although, in theory, the model could learn this itself, 
% $mask_t(n)$ 
% allows us to expedite the process of learning and does \emph{not} spend model capacity for learning a deterministically known fact. 
% This mask is a 0/1 mask over the vocabulary and can be pre-computed.

\subsubsection*{Copying}

In contrast to Yin~\etal, that is learning to generate code given 
natural language as input, we can take advantage of the fact that tokens 
that appear in source $S$ will also appear in target $T$. 
To use this fact, 
we turn to copying mechanisms, originally proposed by Vinyals~\etal~\cite{vinyals2015pointer}. It is a neural architecture to 
learn the conditional probability distribution of an output sequence to 
positions in an input sequence. It uses an attention mechanism as a pointer 
to select input token to be copied to the output sequence. 
The conditional probability of an input token being copied to 
output sequence is given by~\Cref{eqn:ptr-net}. 
Here, $\omega(\phi)$ refers to the function of a deep feed-forward neural network with input $\phi$. Equation~\ref{eqn:ptr-net} gives a probability distribution over all tokens %(positions) 
in the input sequence. We use this probability to add to final probability of an output token. 

Since we are dealing with code changes, not all the tokens from the source should be copied. We wanted to let the model generate some tokens as well. We let the model learn the probability that tells us when to copy. The model calculates that probability as $p(copy_t|S, a_1...a_{t-1})$~\Cref{eqn:copy-prob}.
% \begin{equation}
%     \label{eqn:copy-prob}
%     p(copy_t|S, a_1...a_{t-1}) = softmax(W_C \cdot s_t)
% \end{equation}
% which is the probability of applying copying.
% \sk{describe copying probability
% }as-is (even if $w_t$ has never been seen in training) the token $w_t$ where $\{w1,w2,...,w_n\} \in x$. 
Finally, marginalizing over the two token generation mechanisms together,

\small
\begin{multline}
    p(a_t = InsertToken(v = \hat{v}) | S, a_1...a_{t-1}, n_f^t) \\
            = (1 - p(copy_t|S, a_1...a_{t-1})) * p(v = \hat{v}|S, a_1...a_{t-1}, n_f^t)\\
            + p(copy_t|S, a_1...a_{t-1}) * p(w = \hat{v}|copy, S, a_1a_2...a_{t-1})
\end{multline}

\normalsize 
The probability distribution for action at time $t$ becomes:

\small
\begin{multline}
    p(a_t | S, a_1...a_{t-1}) = \\
    \begin{cases}
    p(a_t = ApplyRule | S,  a_1...a_{t-1}, n_f^t) & \text{if } n_f^t \text{ is non-leaf}\\
    p(a_t = InsertToken | S, a_1...a_{t-1}, n_f^t) & \text{if } n_f^t \text{ is leaf}
    \end{cases}
\end{multline}
\normalsize

%An example of decoding scheme at $t_7$ or figure~\ref{fig:motiv_ed} is embellished in figure~\ref{fig:detailed_step}.

==> backups/rq0_back.tex <==
To develop \tool, we faced many design choices. We start with systematically evaluating them.

\RQ{1}{\rqd}

%In this research question, we systematically investigate different design choices that we faced while designing \tool. We will also see the evolution of \tool's motivation. 

\begin{table}[!htb]
    \centering
    \caption{\textbf{\small Number of correct patch generated by \tokenmodel when actual transformed tree is known.}}
    \label{tab:gold_tree}
    \begin{tabular}{c|c|c}
         \multirow{2}{*}{Dataset} &\multicolumn{2}{c}{ Total Correct Patches}\\
         
          & \sts & \tokenmodel with gold structure\\
         \midrule
         \dataname & 456 (6.67\%) & 1509 (22.09\%)\\
         \icsedata & 33 (3.12\%) & 250 (23.63\%)\\
         \bottomrule
    \end{tabular}
\end{table}

At first, we are interested in investigating whether structural code change help at in the NMT based code change prediction task. We implemented a baseline \sts model and a \tokenmodel model. We assumed that developers already know what kind of structural change developer want to apply (\ie developer already know the actual \tnew). ~\Cref{tab:gold_tree} shows results in these settings. While baseline vanilla \sts can generate 6.67\% (456 out of 6831) and 3.12\% (33 out of 1058) correct patches for \dataname and \icsedata respectively in top 10 positions, with the help of actual \tnew, \tokenmodel model of \tool can generate 22.09\% (1509 out of 6832) and 23.63\% (250 out of 1058) for \dataname and \icsedata respectively. Note that, this is not \tool's final result. This is only an intermediate result that guides the motivation towards \tool development. This results empirically proves that tree structure can improve NMT based code change prediction models' performance significantly.

\begin{table}[!htb]
    \centering
    \caption{\textbf{\small Performance of \treemodel in different datatypes and different form of data}}
    \label{tab:tree_prediction}
    \begin{tabular}{c|c|c}
         \multirow{2}{*}{Dataset} &\multicolumn{2}{c}{ Total Correct Patches}\\
          & Full Dataset & Filtered Dataset\\
         \midrule
         \multirow{2}{*}{\dataname} & 4204 / 6832  & 1271 / 3782 \\
         & (61.54\%) & (33.61\%)\\
         \midrule
         \multirow{2}{*}{\icsedata} & 408 / 1058  & 256 / 833 \\
         & (38.56\%) & (30.73\%)\\
         \bottomrule
    \end{tabular}
\end{table}

Now that we know tree structure boosts performance of NMT based code change models. We wanted to investigate more on designing a model that can learn the structural changes in code and predict structural changes. With that motivation in mind, we designed \treemodel \textemdash~a tree translation model to translate a given tree structure. ~\Cref{tab:tree_prediction} shows the result of correctly predicted trees. \treemodel can perfectly predict tree structure of the next version (\ie \tnew) for 61.54\% and 38.56\% of test examples in \dataname and \icsedata respectively. However, as expected, not all the patched have structural changes. Some patches do not have any structural changes. In particular, 3782 test patches from \dataname, and 833 test patches from \icsedata actually have structural changes. We trained a separate version of \treemodel with the training patches where there is at least 1 node difference between the \tnew and \told.  Also we removed those examples, where there is no structural change from the test example scope. This is out filtered dataset (see ~\Cref{tab:tree_prediction}). In filtered dataset, \treemodel component of \tool can predict 33.61\% and 30.73\% transformed structure from \dataname and \icsedata respectively.


Having \treemodel and \tokenmodel evaluated separately, we are interested in developing a end-to-end model for NMT based code change prediction. We designed \treemodel and \tokenmodel to develop \tool. While designing \tool, we faced some design problem that we will describe in this section. 

\begin{table}[!htb]
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c}
         Dataset & without replace & allow & replace\\
         \midrule
         \multirow{2}{*}{\dataname} & 727 & 1309 & 1075\\
         & 10.64\% & 19.16\% & 15.73\% \\
         \midrule
         \multirow{2}{*}{\icsedata} & 81 & 160 & 138\\
         & 7.66\% & 15.12\% & 13.04\%\\
         \bottomrule
    \end{tabular}
    \caption{Performance in different configuration of \tool. First configuration is vanilla \tool, second configuration is same as vanilla \tool but while evaluating performance, we considered {\tt <unknown>} token to be any token, third configuration is where {\tt <unknown>} token is replaced by source token with highest attention probability.}
    \label{tab:replace_unk_summary}
\end{table}

First, \tokenmodel generates a probability distribution over the vocabulary. Since the vocabulary is generated based on the training data, tokens of test patches that do not exist in vocabulary are replaced by special {\tt <unknown>} token. In fact, our experiment shows \tool generates a lot of patches where {\tt <unknown>} token gets higher probability. And hence the generated code will have {\tt <unknown>} token which does not make any sense (code will not compile and hence is not a valid suggested code). For instance, in our experiment, \tool can predict \textbf{727 (10.64\%)}, and \textbf{81 (7.66\%)}  correct patches in \dataname and \icsedata respectively. However, if we allowed {\tt <unknown>} to be semantically equivalent to any other token, number of correct patches goes up to \textbf{1309 (19.16\%)} and \textbf{160 (15.12\%)} correct patches in \dataname and \icsedata respectively. Albeit this result is not complete result, it shows the need for a method that tackles the problem of {\tt unknown} predicted token. To solve this problem, we replace any {\tt <unknown>} token predicted by \tokenmodel with the source token with the highest attention probability following ~\Cref{eqn:context_token}. With this improvement, \tool can successfully generate \textbf{1075 (15.73\%)}, and \textbf{138 (13.04\%)} correct patches from \dataname and \icsedata respectively. The results are summarized in ~\Cref{tab:replace_unk_summary}.


\begin{table}[!htpb]
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c}
         \multirow{2}{*}{Dataset} & \multicolumn{4}{c}{$K2 = 10$}\\
         & $K1 = 1$ & $K1 = 2$ & $K1 = 5$& $K1 = 10$ \\
         \midrule
         \multirow{2}{*}{\dataname} & 1075 & 1080 & 398 & 518\\
         & 15.73\% & 15.81\% & 5.83\% & 7.58\%\\
         \midrule
         \multirow{2}{*}{\icsedata} & 138 & 152 & 105 & 126\\
         & 13.04\% & 14.37\% & 9.92\% & 11.91\%\\
         \bottomrule
    \end{tabular}
    \caption{Different configurations of $K1$ that are tested on \tool. In both \dataname and \icsedata considering top 2 trees generated by \treemodel, expanding each into 10 different token sequences resulting in 20 probable $c_n$ and then choosing top 10($K$, this is a user input parameter) prospective $c_n$ following ~\Cref{eqn:score_cn}, results in best performing model.}
    \label{tab:k1k2}
\end{table}

Second, we have two configuration parameters, $K1$ and $K2$ \ie number of trees generated by \treemodel and number of token sequences generated by \tokenmodel. ~\Cref{tab:k1k2} shows results for different values of $K1$ and $K2$. With $K = 10$ (user preference), $K1 = 2$, $K2 = 10$, we got the highest performing result in both \dataname and \icsedata. 


% \input{tables/design-choices.tex}

% ~\Cref{tab:tuning} summarizes our different design choices related to abstract and concrete patch generation.

% \input{tables/tuning.tex}

% \noindent
% \textbf{{Abstract Patch.}}
% % First, we had to decide the right level of code abstraction and to suggest changes. 
% We experimented with following code abstractions and models:

% \noindent
% (i) {\textit{\sts + Token}}: 
% We start with simply tokenizing the code. % without considering the identifier types.  
% For example, a code fragment  
% {\tt return fit({{new Gaussian.Parametric(),}} guess)} is expressed as  {\tt return t3 ({{new t1 () ,}} t2 )}. 
% %Every identifier in training and testing dataset is replaced by a symbolic token name. 
% We choose this abstraction because many language models could successfully generate code with this abstraction~\cite{hindle2012naturalness,Tu:2014:FSE,hellendoorn2017deep}.  Then, we applied our vanilla \sts model as described in~\Cref{ref:experiment}. In this setting, we found 300 and 743 correct patches out of 6735 total patches in top 1 and top 10 respectively. 
% %\item

% \noindent
% (ii) {\textit{\sts + Token Type}}: Next, we consider the AST types of the identifier names. For instance, the code fragment shown above %{\tt return fit ( \sout{\Red{new Gaussian.Parametric () ,}} guess ) ; } will be 
% is treated as {\tt return METHOD\_1 ( {{new PACKAGE\_1 () ,}} VAR\_1 )}. 
% %Then we train and test \sts model with this data set.  
% ~\Cref{tab:tuning} shows the result: 444 and 887 correct patches are correctly suggested in top 1 and top 10 respectively. 
% %\item

% \noindent
% (iii) \textit{Tree2Tree + Token.}  Next, we use tree2tree model on abstract code fragment to generate abstract patches.  Depending on the configuration, \tool produces three types of abstract patches: without identifier names (tree only), with abstracted names, and with token types. 
% In first case, \tool only predicts the tree. This allows \tool to predict any structural changes. With this configuration, \tool predicted 2022 patches correctly in top 10. The second configuration consists of dataset where token names are replaced abstract symbolic token names.
% (\ie {\tt t1}, {\tt t2} etc.). 
% With this configuration, \tool predicted  1567 correct patches in top 10. 
% The third and the final configuration consist of a dataset where token names are replaced by token types. 
% In this configuration, \tool predicted 650 correct patches in top 1 and 760 in top 10. 

% Although \tool performs best while predicting only the tree, we choose to present the results with abstracted tokens in rest of the paper as that will give us an opportunity to compare the vanilla \sts model on a fair ground. At this setting, \tool suggests 608 correct abstract patches at top 1 and 1567 correct patches at top 10. 
% %\end{enumerate}


% \noindent
% \textbf{Concrete Patches.}
% With concrete dataset, the vocabulary size explodes. To keep the model tractable, we had to use a threshold of maximum vocabulary size. However, the concrete dataset vocabulary is much larger than that of the maximum vocabulary size. 
% The out of vocabulary tokens are replaced by special {\tt <unknown>} token, similar to most NLP models. When we applied a \textit{no\_copy + no\_mask} setting (See~\Cref{susec:decoder}), 157 correct patches are suggested in both top 1 and top 10. A lot of the patch suggested in this setting had {\tt <unknown>} token in the generated code. 

% Next, with copying technique (see section~\ref{susec:decoder}), \ie \textit{copy + no\_mask},  \tool predicted 225 correct patches in top 1 and 372 in top 10. 
% We further tested \tool with applying a token mask to filter out impossible out-of-scope tokens (\textit{copy + mask}). \tool resulted in slightly better results (\eg 374 correct patches in top 10) than results with (copy + no\_mask). 
% Thus, as a final model for generating concrete patches, we used ``copy + mask'' settings. Note that, the $mask$ we discuss here is not the same mask discussed in section~\ref{sec:model}. Instead, this token mask depends on the type of the terminal node and is statically pre-computed.

% \begin{table}[!htb]
%     \centering
%     \scriptsize
%     \caption{\textbf{\small Percentage of correct abstract test patches generated by \tool with varied beam sizes.\vspace{-10pt}}}
%     %\begin{tabular}{l|c|c|c|c|c}
%     \begin{tabular}{lccccc}
%         \toprule
%          Trained  &  \multicolumn{5}{c}{\% of correct patches in Top}  \\
%          \cline{2-6}
%          Model Type  & 1 & 2 & 5 & 10 & 20\\
%          \midrule
%          $Model_{ppl}$ & 8.29 & 11.58 & \textbf{20.04} & 23.1 & 26.16\\
%          \midrule
%          $Model_{bl}$ & \textbf{9.03} & \textbf{14.54} & 19.90 & \textbf{23.27} & \textbf{26.53}\\
%          \bottomrule

%     \end{tabular}
%     \label{tab:abs-res-summary}
% \end{table}

% We further evaluate \tool's ability to suggest  correct abstract patches \wrt two models: 
% (i) the model with best perplexity ($Model_{ppl}$) in validation dataset, 
% (ii) the model with best BLEU in validation dataset ($Model_{bl}$).
% ~\Cref{tab:abs-res-summary} shows the percentage of correct patches generated by the two models. 

 

% Although, the two models perform similarly, $Model_{bl}$ performs slightly better than $Model_{ppl}$. Thus, in subsequent evaluations of this paper, we use $Model_{bl}$. 

% \RS{1}{A Tree-to-Tree model works best for abstract patch generation and for concrete patch generation it works better with copying and masking technique.}


==> backups/rq1.tex <==
%!Tex root=./main.tex

% With the best performing settings, next we evaluate: 
Let us first focus on how \tool is preforming in compare to other baseline. 

\RQ{2}{\rqa}

% ~\sk{Baishakhi: this whole para should go in expreiment design.
%  To answer this research question, we first analyzed our patches $(AST_b, AST_a)$~\ref{subsec:data-col}, and created a symbol table. In the symbol table, each object and class names are replaced by a symbolic name, and in the symbol table corresponding original name is stored. Thus we have patch trees that retain the structural changes in the original patch putting less emphasis on predicting tokens. Similar method of abstracting away the tokens is adopted by Tufano~\etal~\cite{tufano2018nmt_bug_fix}.}
 
To evaluate this RQ, we evaluate \tool's accuracy \wrt to a data set containing abstract patches (\ie with abstracting away the identifier names).~\Cref{tab:abstract} shows the result.
\tool can correctly generate 608, 979, 1340, 1567, and 1787 abstract patches out of 6735 total patches with beam size 1, 2, 5, 10 and 20 respectively. Thus, \tool can generate up to 26.53\% abstract patches with beam size 20. 

\input{tables/abstract.tex}

\noindent
\textbf{\tool vs.~\sts.} We further compare \tool's performance to generate abstract patches with a vanilla \sts model, as described in~\ref{subsec:baseline}.
~\Cref{tab:abstract} shows the result. Across all the beam sizes, \tool performs significantly better than the \sts model. 
For instance, at Top 1, \tool finds the correct patch with 9.03\% accuracy, while \sts has 4.45\% accuracy. The difference increases further with larger beam size. For example, at beam size 20, \tool 's accuracy is 26.46\% while \sts's accuracy is only 13.43\% respectively. 
Thus, overall, we see a gain of around  103\%, 194\%, 175\%, 110\%, and 97\% at beam sizes 1, 2, 5, 10 and 20 respectively. 



%Now, let's look at some of the qualitative examples that are generated by \tool. 
Table~\ref{tab:examples} further shows some examples to illustrate the difference between the two models. Note that, as described in section~\ref{subsec:baseline}, here our baseline is a vanilla \sts model that works on a sequence of tokens. Thus, we also asked \tool to produce patches with the same abstraction, for fair comparison.

Ex1 shows an instance of statement deletion that \tool is able to successfully suggest . The \sts model suggested a patch, which is syntactically correct but not the right patch. In case of Ex2, both \tool and \sts successfully generated correct patch. Ex3 shows a patch where \sts could generate successful patch but \tool could not. The best \tool did here removing the parameter from {\tt t2}'s constructor. However, the correct patch contains a different API {\tt t3}. 
%In example 2 however, the \seq model generates a code that is not syntactically correct. Although, it is apparent from the code that {\tt t7} is a data type name, \seq model generated it in place of a variable name. 
%As a natural language model, neither \tool nor \seq has any information about {\tt t7}(whether it is a data type or it is a variable name). However, since \tool is built on parse tree structure in contrast to the sequence, it has some additional information over the \seq model. 
%Example 3 is an example of API change, where {\tt t3}(a class constructor) is not taking any parameters. Both \tool and \seq generated correct patch in this case. This is a fairly easy example for \seq model since it involves deleting some tokens. Although both \tool and \seq model generated the correct  change, \tool placed it correct patch in $8^{th}$ position and \seq placed this patch in $4^{th}$ position in respective rank list, since this change involves more work for \tool than \seq, \seq performed better than \tool in this case. 
% Other type of model applicable here could be entity-composite model that takes in the type information of a variable along with the context.  

\input{tables/abstract_examples.tex}

\medskip
\noindent
\textbf{Variation of performance with edit size.} 
We further noticed that, with different edit sizes \tool's performance varies. 
%For instance, one could expect \tool will perform better when  only one node is changed in the source tree (\ie edit size=1). 
To estimate how \tool's performance varies with edit sizes, for each patch in our test dataset, we calculate the tree edit distance between the corresponding source and target tree~\cite{pawlik2016tree, pawlik2015efficient}. 
We then divide the distances into 3 bins:  ({\em small}: $edit\_{size} = 1$, {\em medium}: $2 \le edit\_{size} \le 5$, and {\em large}: $6 \le edit\_{size} \le 10$) and analyze the \tool's performance. As shown in~\Cref{tab:abstract}, 
\tool performs better at smaller edit sizes. For example, at beam size 20, for $edit\_size=1$, \tool correctly suggests $1358$ edits out of total $3368$ edits ($40.32$\%  accuracy). In contrast, at the same beam size, the \tool's accuracies at medium and large edit sizes are: 11.01\% and 15.46\% respectively. Similar trend is observed across all the beam sizes and also for the \sts model.

\begin{figure}[htpb]
  \includegraphics[width=0.9\columnwidth]{images/abstract_edit.pdf}
  \label{fig:abs_edit}
\caption{\textbf{\small{Variation of performance with edit sizes.  The figure shows a cumulative plot of how the percentage of correct (abstract) patches vary with different edit sizes across different beam sizes. All the percentage numbers are calculated \wrt total patches. }}\vspace{-10pt}}
\label{fig:abs_ed}
\vspace{-5pt}
\end{figure}

~\Cref{fig:abs_ed} further shows the variation of accuracy with edit sizes using a cumulative plot. Here, the accuracy at each edit size are measured \wrt the total patches in the evaluation set.  The figure shows that at beam size 1 (orange lines),  the accuracy of \tool  is $8.61$\% and then remains almost constant with the larger edit sizes. 
In contrast, at beam size 20 (blue lines), \tool starts with an accuracy of 20.11\% and then gains slowly up to 26.26\% for edit size 10. It gains steadily till edit size 3, and then almost remains flat till edit size 7.  It again gains accuracy at edit size 8 and then remains almost constant after that.  
\tool  follows a similar trend for beam size  5. 
% ~\sk{Explain the gain at edit size 8}.
There is a sudden boost in performance at edit size 8. 
We surprisingly found that, a large number of candidate patches in our test dataset 
are of same type. \tool could successfully suggest all those edits. 
\sts model have a similar trend but at a much lower rate. Thus, we see          that, in general, \tool is better suited for suggesting  smaller patches (1-3 edit sizes) rather than the larger ones.

Since we are performing well at smaller edit sizes, one could imagine that we are only good at suggesting trivial changes. To check that we ignore the patches with token renaming and then compare \tool's accuracy with the rest of the patches (3439 in total). 
We find that we could still predict 9.68\% to 18.32\% patches from beam size 1 to 20.  

These results prove that \tool can suggest abstract patches with good accuracy. Such patches can be used by the developers as change 
templates (similar to refactoring templates provided by modern IDEs). 

% \RS{2}{\tool can suggest abstract changes with accuracy up to 26\% and outperforms baseline \sts model with a large margin.}
\RS{2}{\tool can suggest 26\% of the abstract changes at top 20 and significantly outperforms its \sts alternative. For single node changes, \tool can correctly suggest as much as 40\% patches.}



==> backups/rq1_bck.tex <==


To answer this RQ, we evaluate \tool's accuracy \wrt the evaluation dataset containing concrete patches. Table~\ref{tab:concrete} shows the results: 
for \dataname dataset, \tool can successfully generate $423$ ($6.19$\%), $788$ ($11.51$\%), $860$ ($12.59$\%), and $1080$ ($15.81$\%) patches.
%\tool achieves 6.19\%, 11.51\%, 12.59\%, and 15.81\% accuracy in suggesting top 1, 2, 5, 10  patches respectively. 
We further compared the results generated by \tool with a \seq model, as described in~\Cref{sec:experiment}. 
Both the models are trained on the same training data.
%On the other hand, \sts alternative solution of code suggestion tool (similar to the one proposed by Tufano~\etal~\cite{tufano2019learning}) 
\sts model suggests 5.13\%, 6.00\%, 7.14\%, and 7.97\% correct patches in top 1, 2, 5, and 10. This shows \tool is outperforming its \sts alternative by 16.5\%, 92.20\%, 76.23\%, and 98.16\% in suggesting concrete patches at top 1, 2, 5, and 10 respectively. 
%Among the patches generated correctly at top 10 by \tool, x\% 
%~\sk{top 1 difference is not too high. Should we report it at all?}
Similar result is observed for \icsedata as well, as shown in~\Cref{tab:concrete}.

\input{tables/concrete.tex}

To further understand the kind of patches we can generate, 
we manually looked at the successfully generated patches at top 10 by each model from \dataname dataset. We manually categorize these patches into 50 categories. 
Two authors individually categorized them and then resolved the conflicts, if any, by discussion. These 50 categories are then further combined into 13  coarse-grained patch types, as described in~\Cref{fig:change_category}. The Figure gives us a detailed insight into the kind of patches \tool can generate, and how it compares with baseline \sts. 

\begin{center}
\noindent\begin{minipage}{0.95\linewidth}
% \includegraphics[width=6cm]{images/Change-Categories.pdf}
% \captionof{figure}{Example figure caption (non-floating)}
% \label{fig:examplenf}
\includegraphics[width=0.95\textwidth]{images/patch_type.pdf}
%\captionof{table}{Example Table (non-floating)}
{\scriptsize
 %\setlength{\tabcolsep}{1pt}
 %\renewcommand*{\arraystretch}{1}
\begin{tabular}{l|p{0.65\textwidth}}
    \toprule
    \textbf{Change Type} & \textbf{Description} (See \Cref{tab:concrete_examples} for examples)\\
    \midrule
    API  & Modify API and Method Call (Example-1) \\
    Type  & Change of Types (Example-2) \\
    Parameter & Add/delete/modify/reorder method parameters (Example-3) \\
    Refactor & Bracketing, variable or method renaming, etc. (Example-4) \\
    Object Reference & Changes in Object or Class Reference (Example-5)\\
    Statement Related & Addition, Deletion, Change of statements.  (Example-6)\\
    Inheritance & Add/delete abstract keyword, super() call, @Override  (Example-7)\\
    Exception & Modify related to Catch, Throw, and other exceptions (Example-8)\\
    Other Changes & Conditions, Values, Data-dependency, etc. (Example-9)\\
    Final & Add/delete final keyword (Example-10)\\ 
    Access & Modify Access Type (\eg public, private, protected) (Example-11)\\
    Annotation & Add/delete Nullable \\%before variable, methods and parameter \\
    %\midrule
     %in methods \\
    %\midrule
    
   % \midrule
    %in methods, parameter and/or variables \\
    %\midrule
    
    %\midrule
    % Method Call & Add/delete or Changes in Methods call \\
    %\midrule
    
    %\midrule
    
    %\midrule
    
    %\midrule
    
    %\midrule
    
    %\midrule
     %Change array type argument to variable length argument, etc. \\
    \bottomrule
\end{tabular}
}
\captionof{figure}{\textbf{\small Patch types successfully suggested by \tool, \sts, and both the models at top-10. The table describes each type of changes.}}    \label{fig:change_category}
\end{minipage} 
\vspace{0.2cm}
\end{center}







%In particular, we divide the number of patches in each type into three bins: only \tool is successful, only \sts is successful, and both are successful in generating the correct patches. 

% First and foremost, we wanted to understand what kind of patches \tool can generate and how those patch categories are similar and dissimilar to baseline \sts model. In order for doing that, we manually classify patches into 50 categories. Two authors individually manually classified those. After analyzing each of the category and corresponding patches, we further combined categories into 12 coarse grained patch type bins based on the patches types. Note that, this coarse grained comparison will give us more detailed insight of the kind of patch that \tool can generate. ~\Cref{fig:change_category} shows number of patches in each path type into 3(three) different bins : \ie number of patches where only \tool is successful, only \sts is successful and both are successful to generate correct patch. \tool performs very well in `API related' patches. This coarse grained patch category includes changing API, calling different methods from and object etc. 'Object Reference' change, on the other hand includes patches where a method/member variable is accessed from different object. Similar to these patch categories, in `Method Call' category, both performs reasonably well. This category corresponds to the changing method call from the same class. 

% Patch category `Annotation' comprises of addition and deletion of annotation before methods, parameters, and variables. In some patches, method access type modifiers (\javaKeyWord{public}, \javaKeyWord{private}, \javaKeyWord{protected}) are changed. Those patches are summarized in `Access' category. Category `Exception' consists of patches changing Exception type, catching different Exception etc. Patches in `Final' categories are addition or removal of \javaKeyWord{final} keywords from methods, parameters, or variables. `Inheritance' category includes patches that adds/removes {\tt @Override} annotation, add/remove \javaKeyWord{abstract} keyword, add \javaKeyWord{super}() call to the parent class's constructor. Our experiment result shows that \sts could not  add  \javaKeyWord{super}() call to any of the given examples, \tool, however, adds  \javaKeyWord{super}() call if a constructor is given to it. Since, \tool does not have any knowledge about the parent class (also its constructor), \tool sometimes adds this  \javaKeyWord{super}() call with wrong parameters. However, we believe, further research combining machine learning and concrete program analysis will help us solve these kind of problems. 

% The `Parameter' change category consists of patches where method parameters are added, deleted, changed, reordered. Category `Refactor' refers to patches with bracekting, renaming etc. `Statemet Related' patches are where statements are added and deleted. \sts works very well in deleting statements, \tool, on the other hand works reasonably well in both adding and deleting statement. `Type Related' patches include changing type in variable declaration, parameter declaration etc. There are some fine grained categories where we have relatively fewer number of patches. We combine those patches to `other' category. These patches include \emph{change in boolean value} (\ie \javaKeyWord{true} to \javaKeyWord{false} or vice versa), change in conditional statement, changes in initialization, changing array type argument to variable length argument etc. 

Here, we can see that \tool is performing significantly higher than \sts in suggesting `API related' changes. In particular, \tool was able to suggest 257 correct changes at top 10. In contrast, \sts was able to predict 33 correct patches. The main reason lies in the structure of \sts and \tool. In \sts, while predicting token (\ie API name), the model generates a probability distribution over all the possible token. On the other hand, since \tool already knew the type of the token it was predicting (from \treemodel), the search space is reduced significantly. One example patch where \tool can successfully generate in top 10 is shown by Example 1 in~\Cref{tab:concrete_examples}. Such reasoning also holds for `Type Changes' and `Object Reference Changes' (see example 2 and 3 in ~\Cref{tab:concrete_examples}).
In Exception related patch category, patches reflect structural changes, as well as change of catching different type of exceptions. \tool can successfully suggest all the patches that are suggested by \sts. In addition to those, \tool can successfully generate non-trivial patches where the patch involves structural change. One such example is shown in~\Cref{tab:concrete_examples} Example 4. Here, first 2 statements are put into a \javaKeyWord{try} block and last statement is put into \javaKeyWord{finally} block. 

\input{tables/concrete_examples}

Both \tool and \sts does reasonably well while adding or deleting parameter to method call. Example 5 (delete method parameter), and Example 6 (add method parameter) in ~\Cref{tab:concrete_examples} shows two successful patches that belong to this category. In `Inheritance' category, most of the successful patches generated by \sts are addition or deletion of {\tt @Override} annotation. However, in \tool can predict some non-trivial patches. For example, in Example 7, \tool does not only add \javaKeyWord{abstract} keyword in method signature, it also removes the body. Since, \tool is built on PCFG, \tool learns that the probability of a method declaration node expanded with a rule having both \javaKeyWord{abstract} keyword and method body is very low. 

Both \tool and \sts does reasonably well in changing the access type modifiers (\eg \javaKeyWord{public}, \javaKeyWord{private}, \javaKeyWord{protected}). Example 8 shows such an example patch where a \javaKeyWord{public} constructor was changed to \javaKeyWord{protected}. Being a tree based model, \tool is very good at capturing the long distance (\ie structural) dependency. Hence, \tool performs well in refactoring. Example 9 in ~\Cref{tab:concrete_examples} shows example where method parameter {\tt x} is renamed to {\tt session}, on top of that this renaming is reflected in the method body. \tool can also learn to add statements from the training data. Example 11 shows an example where \tool adds {\tt Thread.interrupted();} statement after the code and before the end of the method. 

% \sk{New similar change results are in tables/similar_change_examples}

\input{tables/similar_change_examples}

Despite these successes in these categories, \tool has some limitations. If the tree corresponding to the correct patch in not predicted within top \ktree by \treemodel, \tool cannot generate correct patch. For instance, in Annotation category, the transformed tree that corresponds to the correct patches are not predicted in top \ktree positions by \treemodel. Hence, \tool failed to predict correct patches in this case. 













To further understand what kind of patches \tool can generate, we further looked at the individual patches generated by each of the model quantitatively and qualitatively analyze the patches generated by both the models. 
First, we qualitatively analyze the patches and assigned a patch class to identify 
In particular, we measure (i) \tool's performance \wrt patch size, (ii) patch type.




To further understand what kind of patches \tool can generate, we quantitatively and qualitatively analyze the patches generated by both the models. 
First, we qualitatively analyze the patches and assigned a patch class to identify 
In particular, we measure (i) \tool's performance \wrt patch size, (ii) patch type.   

\noindent
\textit{Patch Size.} 
To look better into the \tool's capability, we do a quantitative investigation on correctly generated patches from both \dataname and \icsedata. First, we are interested in seeing how large are the correctly generated patches are. To measure the size of the patch we used two different metric. Our first metric is Edit distance between the previous version of code (\cold) and the generated code (\cnew). \Cref{fig:ed_hist} shows the histogram of token diff size ($\Delta_c$). We measure $\Delta_c$ in terms of edit distance~\cite{masek1980faster} between \cold and \cnew. \tool performs well to generate small diff sizes \ie $\Delta_{c} \leq 4$ token changes for \dataname and $\Delta_{c} \leq 10$ for \icsedata. However, \tool can also generate successful patches for larger diff sizes.  For instance, ~\Cref{fig:ed_hist_codit} shows a spike in $\Delta_c = 8$ (see ~\Cref{fig:ed_hist_codit}). 
% \rayb{This histograms are rather skewed towards smaller changes. However, this skewness is contribution of many factors along with \tool's performance, \ie distribution in data, change type etc. I do not know how to rationalize this skewness \ie to me, if I read this, it leaves a question mark.}

Here, we analyze what size of patches \tool can successfully generate.  
We measure the patch size in terms of edit distance between the previous and new version of the code. Since \tool operates on both token sequence and tree structure, we show the results using both token-based  (\Cref{fig:ed_hist}) and tree-based edit distances (\Cref{fig:td_hist}). 
These figures show the histogram of patch size generated by \tool. 

~\sk{I need the percentage patch size per bin to say tool perform better}.
To look better into the \tool's capability, we do a quantitative investigation on correctly generated patches from both \dataname and \icsedata. First, we are interested in seeing how large are the correctly generated patches are. To measure the size of the patch we used two different metric. Our first metric is Edit distance between the previous version of code (\cold) and the generated code (\cnew). \Cref{fig:ed_hist} shows the histogram of token diff size ($\Delta_c$). We measure $\Delta_c$ in terms of edit distance~\cite{masek1980faster} between \cold and \cnew. \tool performs well to generate small diff sizes \ie $\Delta_{c} \leq 4$ token changes for \dataname and $\Delta_{c} \leq 10$ for \icsedata. However, \tool can also generate successful patches for larger diff sizes.  For instance, ~\Cref{fig:ed_hist_codit} shows a spike in $\Delta_c = 8$ (see ~\Cref{fig:ed_hist_codit}). 
% \rayb{This histograms are rather skewed towards smaller changes. However, this skewness is contribution of many factors along with \tool's performance, \ie distribution in data, change type etc. I do not know how to rationalize this skewness \ie to me, if I read this, it leaves a question mark.}


\begin{figure}[!htpb]
    \centering
    \subfigure[\textbf{\dataname}]{
    \includegraphics[width=0.45\textwidth]{images/patch-size-hist/edit-size-hist-edit-dist-codit.pdf}
    \label{fig:ed_hist_codit}
    }
    \subfigure[\textbf{\icsedata}]{
    \includegraphics[width=0.45\textwidth]{images/patch-size-hist/edit-size-hist-edit-dist-icse.pdf}
    \label{fig:ed_hist_icse}
    }
    \caption{Patch size (Token Edit-distance) histogram of correctly generated patches in different datasets.}~\sk{Increase font}
    \label{fig:ed_hist}
\end{figure}


Next, since \tool is a tree based model, we investigate the difference between the given tree (\told) and successfully generated tree(\tnew). We measure different between \told and \tnew ($\Delta_t$) in terms of tree edit distance~\cite{pawlik2016tree, pawlik2015efficient}. \Cref{fig:td_hist} shows the histogram of $\Delta_t$. Here, we also see that \tool is very good at generating smaller changes. For instance, \cref{fig:td_hist_codit} shows, \tool generate successful patches for $\Delta_t \leq 4$ in \dataname. In \icsedata, \tool generated successful patches for larger tree distance. \Cref{fig:td_hist_icse} shows that \tool generate few successful patches where $25 \leq \Delta_t \leq 30$.  
\begin{figure}[!htpb]
    \centering
    \subfigure[\textbf{\dataname}]{
    \includegraphics[width=0.45\textwidth]{images/patch-size-hist/edit-size-hist-codit.pdf}
    \label{fig:td_hist_codit}
    }
    \subfigure[\textbf{\icsedata}]{
    \includegraphics[width=0.45\textwidth]{images/patch-size-hist/edit-size-hist-icse.pdf}
    \label{fig:td_hist_icse}
    }
    \caption{Patch size (Tree Edit Distance) histogram of correctly generated patches in different datasets.}~\sk{remove legend}
    \label{fig:td_hist}
\end{figure}

\noindent
\textit{Patch Type.}



% Let us now focus on, some qualitative samples of change type that \tool can successfully generate patches. 
% ~\sk{Can you summarize AST parent node types per patch? Otherwise, following becomes a laundry list.}
% \Cref{tab:concrete_examples} shows some interesting examples showing the correctly generated patches by \tool. 
% \tool can both add parameters to an existing method call and remove parameter from method call. Example 1 is an example of adding method parameter and Example 2 shows an patch where parameter is removed. Example 3 shows an interesting non-trivial patch where three statements are sequentially written in the previous version. \tool generates a patch in top 10 patches (correct patch position 6). The patch encompassed first two statements in a \javaKeyWord{try} block and puts the last statement in \javaKeyWord{finally} block. Example 4 shows a patch where a un-referenced variable is removed. In the previous version of the code, a variable {\tt aa} is initiated which never used inside the scope of that variable. In the next version, assignment of that variable is omitted \ie variable reference {\tt aa} is not created. 

% Examples 5 shows an example, where, in previous version of the code, method did nothing but throwing a {\tt MustOverrideException}, which says the method {\tt removeSessionCookies} has not been implemented here and must be implemented by any child class that extends this class. Implicitly this method is equivalent to an {\tt abstract} method. \tool learns to change this method to abstract method from the training data. Note that, tool does not only add \javaKeyWord{abstract} keyword in method signature, it also removes the body. Since, \tool is built on PCFG, \tool learns that the probability of a method declaration node expanded with a rule having both \javaKeyWord{abstract} keyword and method body is very low. Example 6 makes the parameter of the method final. This change makes the parameter immutable. In example 7. {\tt f.createJsonParser( ... )} method call is replaced by {\tt f.createParser( ... )} method call. This is an example of API change. Example 8 shows a refactoring change. Here method parameter {\tt x} is changed to {\tt session}. \tool can not only change the name of the parameter, it successfully applies chat change (\ie replace {\tt x} with {\tt sesstion}) in method body. 



 

% \begin{figure}[!htpb]
%     \centering
%     \small
%     \includegraphics[width=0.95\textwidth]{images/near-miss.pdf}
%     \caption{\small{\textbf{\tool's performance in near-miss patch suggestion. x-axis shows the edit-distance from the actual patch and y-axis shows the cumulative percentage of patches.}}}
%     \label{fig:near_miss}
% \end{figure}
% ~\sk{I think we should give normalised distance than exact distance will make more sense. I will do this change first thing tomorrow morning, the data is in office desktop.}
% Since \tool is a patch suggestion tool, predicting exact patch is not always necessary, developers have to investigate the predicted patches anyway. To investigate how \tool is performing in predicting slightly different patches than exact expected patch, we take the top 1 patch suggestion and calculated how similar those patches are in terms of edit distance. We set the edit distance threshold for near-miss patch 3, \ie we are considering recommended patches which at most 3 token different from the correct patch. ~\Cref{fig:near_miss} shows near-miss patches generated by \tool in  top 1. \tool can generate 44.72\% near-miss patch for  \dataname and 27.70\% for \icsedata. Note that, edit distance 0 means patches which are exactly same as developer provided patches. 


% \rayb{Saikat says: I don't know the following paragraph is appropriate or not. But I want to convey the message.}
% We acknowledge that these near-miss patches might be very difficult for the developers to apply. However, sophisticated program analysis based technique can help us transforming these near patches to actual developer provided patches. That's a different problem and beyond this research's scope. We leave investigation of those kind of transformation for future research.  


% ~\Cref{tab:concrete_examples} shows some examples where \tool can successfully generate the concrete patches. For instance, in Ex1, \tool successfully removes a typecasting {\tt CraftInventory}. In Ex2, \tool removes a whole statement from the {\tt if block}. Ex3 and Ex4 further show cases where \tool successfully adds a parameter {\tt true} to a method call and adds a generic respectively. 

% To gain a better insight of the kind of patch \tool can successfully generate, we further investigate the cases where \tool could predict correct concrete patches but \sts could not\textemdash there are 216 such cases at beam size 20.  
% We manually investigated all those patches and assigned a category of the patch considering the change type. 
% The categorization was done by two authors. The lead author first assigned the category, and then another author reviewed them. In case of disagreement, they discussed and came to an agreement. 
% Table~\ref{tab:patch_case_study} shows the results. 

% \input{tables/case_study.tex}

% We notice that the most common patches are related to {\tt final} keywords: 77 times \tool could successfully add or remove them. 
% The next highest category is related to change to method parameters (see Ex3 in~\Cref{tab:concrete_examples}). 
% The other categories are related to changing types, method modifier, and APIs. In total, \tool successfully generated patches in 9 different categories. This results show \tool is applicable to different types of edits. 

% Inspite of these successes, performances of both \tool and \seq model are much lower than that on the abstract dataset because while with concrete dataset the models face an explosion of vocabulary (vocab size around 32000 in original dataset and ~118 in abstract dataset). The token names in concrete edits are so diverse that, even with copying mechanism \tool achieved lower performance.
% For instance, 
% {\tt decrStackSize ( k , \sout{\red{itemsToExtract ()}} \green{count} )} was incorrectly predicted as 
% {\tt decrStackSize ( k , \sout{\red{itemsToExtract ()}}  \green{k} )}, while the corresponding abstract patch %{\tt return t5 . t1 ( t3 , \sout{\Red{t4 ()}} \Green{t2}) ;} 
% was suggested correctly.% by abstract model.

% Thus, it is often the case that the variable name \tool has generated is incorrect, however the rest of the patch is fine. 
% To estimate how far we are from generating the correct concrete patches, we further compute {\em patch distance}: 
% edit distance between a patch produced by an NMT model and the ground truth. Such patch distance can be an estimate of developers' effort to fix the {\em near-miss} patches (\eg patch distance $1$ means developers have to add/delete/change only 1 token).~\Cref{fig:pd} shows the result up to patch distance 5. 

% \begin{figure}[!htpb]
%   \includegraphics[width=0.9\columnwidth]{images/concrete_patch_distance.pdf}
%   \label{fig:pd}
% \caption{\textbf{\small{Histogram of Patch distances (distances between the model generated and ground truth patches)}}\vspace{-10pt}}
% \label{fig:pd}
% \vspace{-5pt}
% \end{figure}

% While \tool can generate only 5\% patches correctly (patch distance=0) at top 5, there are 18\% and 9\% patches that are withing $1$ and $2$ patch distances from the ground truth. Compared to \sts model, \tool can generate around two times more patches within patch distance 1 (659 in case of \seq and 1204 in case of \tool). 
% % For instance, \tool predicted
% % \vspace{2pt}
% % \begin{lstlisting}
% % try { run ( configuration , @\Green{configuration ,}@ params ) ; } 
% % finally { environment . stop () ; }
% % \end{lstlisting}
% % although the correct patch is,
% % \vspace{2pt}
% % \begin{lstlisting}
% % try { run ( configuration , @\Green{environment ,}@ params ) ; } 
% % finally { environment . stop () ; }
% % \end{lstlisting} %\\
% % This is a near-miss patch. However, it is easy for developer to fix it. 
% % \lstinline[language=java]{try\{ run\(configuration, environment, params\);\} finally\{ environment.stop \(\) ;\}}
% % \lstinline[language=java]{if}
% Overall, \tool can generate around 28\% of near-miss patches within patch distance 1 and 2; we believe these patches can be easily adapted by the developers. 



%Till now, we talked about perfectly correct prediction of patch. Since \tool is recommendation tool, it is not always needed to recommend the exact right change. Developers anyway have to investigate the recommended changes before applying those to code-base. While investigating, developer might have to do some minor modifications. Let us investigate the recommended patches from both \tool and \seq model in depth and estimate how much effort is needed to apply the patches. We calculate the edit distance of the recommended code from the actual target code and use that as a simplified proxy of developer effort. We call this distance as patch distance. 
%Figure~\ref{fig:pd} shows minimum edit distance of the recommended codes from the correct target code in horizontal axis and percentage of patches in vertical axis. Patch distance 0 corresponds to the exact match with the correct patch which is detailed in table~\ref{tab:concrete}. \tool brings almost twice as much code as \seq model at patch distance 1 (659 in case of \seq and 1204 in case of \tool). Which implies developers have to  add/delete/change only 1 token in twice as many cases if they deploy \tool as change recommendation tool in contrast to \seq model.




==> backups/rq3-defects4j-backup.tex <==

We evaluate this RQ with the state-of-the-art bug-repair dataset, \defj~\cite{just2014defects4j} using all six projects.
% Since we are interested in testing the viability of using \tool for bug-fix patches, we assumed the bug-fix locations are already given to us as an input.  

\noindent
\textit{\textbf{Training:~}}  We collect commits from the projects' original GitHub repositories and preprocess them as described in~\Cref{sec:approach}. We further remove the \defj bug fix patches and use the rest of the patches to train and validate \tool. 

\noindent
\textit{\textbf{Testing:~}}We extract the methods corresponding to the bug location(s) from the buggy-versions of \defj. A bug can have fixes across multiple methods.  We consider each method as candidates for testing and extract their ASTs. We then filter out the methods that are not within our accepted tree sizes. In this way, we get 117 buggy method ASTs corresponding to 80 bugs. The rest of the bugs are ignored. 

Here we assume that a fault-localization technique already localizes the bug~\cite{abreu2007accuracy}. In general, fault-localization is an integral part of program repair. However, in this paper, we focus on evaluating \tool's ability to produce patches rather than an end-to-end repair tool. Since fault localization and fixing are methodologically independent, we assume that bug location is given and evaluate whether \tool can produce the correct patch. Evaluation of \tool's promise as a full-fledged bug repair tool remains for future work. 

For a buggy method, we extract \cold. Then for a given \cold, we run \tool and generate a ranked list of generated code fragments (\cnew). We then try to patch the buggy code with the generated fragments following the rank order, until the bug-triggering test passes. If the test case passes, we mark it a potential patch and recommend it to developers. We set a specific time budget for the patch generation and testing. For qualitative evaluation, we additionally investigate manually the patches that pass the triggering test cases to evaluate the semantic equivalence with the developer-provided patches. 
Here we set the maximum time budget for each buggy method to 1 hour. We believe this is a reasonable threshold as previous repair tools (\eg Elixir~\cite{saha2017elixir}) set 90 minutes for generating patches. 
SimFix~\cite{jiang2018shaping} set 5 hours as their time out for generating patches and running test cases.

% For each buggy method in our test set, we extract the buggy previous code version (\cold) and its corresponding tree representation (\told). For each \cold, we generate list of generated codes (\cnew). 
% We apply the newly generated code in place of the \cold one by one, then we do additional modification~\sk{give example of modification} to the code to fit in the context where we are applying the patch. 
% For each patch, we run the bug-triggering test cases given by Defects4J. If the test case pass, we call it a success. 
% We set a specific time budget for patch generation and testing. 
% For qualitative evaluation, we further manually investigate the patches that passed the triggering test cases to evaluate the semantic similarity with the developer provided patches. 
%\vspace{-0.2cm}
\begin{figure}[!htpb]
    \centering
    \includegraphics[width=0.75\textwidth]{images/defj-test-patch.pdf}
    \vspace{-0.5cm}
    \caption{\small{\textbf{Patches passing the bug-triggering tests \vs time.}}}
    \label{fig:defj-graph}
    \vspace{-2mm}
\end{figure}
%\vspace{-5mm}

 
\input{tables/d4j}

\tool can successfully generate at least 1 patch that passes the triggering test case for 51 methods out of 117 buggy methods from 30 bugs, \ie 43.59\% buggy methods are potentially fixed.
\Cref{fig:defj-graph} shows the number of patches passing the bug-triggering test case \wrt time. We see that, 48 out of 51 successful patches are generated within 20 minutes. 
%, \tool generate at least 1 trigger test case passing patch.

We further manually compare the patches with the developer-provided patches: among 51 potential patches, 30 patches are identical and come from 25 different bug ids (See Table~\ref{tab:defj_res}). %semantically similar 
%to the developer provided patch. 
%These 30 corresponds to buggy methods from 25 different bug ids. 
%shows all patches identical to developer provided patches that \tool can successfully generate. 
%All the underlying buggy methods of the bugs marked in~\Greenul{green} are successfully fixed by \tool. 
The bugs marked in~\Greenul{green} are completely fixed by \tool with all their buggy methods being successfully fixed. 
For example, Math-49 has 4 buggy methods, \tool fixes all four. 
For the bugs marked in~\blued{blue}, \tool fixes all the methods that are in scope. For example, for Lang-4, there are 2 methods to be fixed, 1 of them are in \tool's scope, and \tool fixes that. 
However, for two other bugs (marked in~\Orange{orange}), 
\tool produces only a partial fix. For example, in the case of Math-46 and Mockito-6, although all the methods are within scope, \tool could fix 1 out of 2 and 2 out of 20 methods respectively.  
The `Patch Type' column further shows the type of change patterns.

We further compare \tool with baseline \sts model (\Cref{subsec:baseline}). 
%To understand \tool's capability, we also use the baseline \sts model (\Cref{subsec:baseline}) 
%trained and test on same dataset as \tool. 
\sts model generates 5 complete and 2 partial patches. Among those 7 patches, \tool generates 6. For Chart-1, \sts generates the fix, but \tool could not. \tool failed to generate this patch because, the correct tree that corresponds to the fixed code was not generated and tested by \tool within the time limit we set. 
% is not generated in top \ktree by \treemodel.

% ~\sk{check these patch types match with previous patch type}.
% \sk{I think we need a table summarizing the numbers}.
% \sk{give some insights about the bugs we cannot fix.}

% One prominent approach in generating and validating~\cite{qi2015analysis} bug repair tools~\cite{saha2017elixir, kim2013automatic} is to transform a suspicious program element following some change patterns until a patch that passes the test cases is found. 
% For instance, Elixir~\cite{saha2017elixir} used 8 predefined code transformation patterns and applied those. In fact, \tool can generate fixes for 8 bugs out of 26 bugs that are fixed by Elixir~\cite{saha2017elixir}.
One prominent bug repair approach~\cite{qi2015analysis,saha2017elixir, kim2013automatic} is to transform a suspicious program element following some change patterns until a patch that passes the test cases is found. 
For instance, Elixir~\cite{saha2017elixir} used 8 predefined code transformation patterns and applied those. In fact, \tool can generate fixes for 8 bugs out of 26 bugs that are fixed by Elixir~\cite{saha2017elixir}.
%
% ~\sk{compare with \sts and simfix, if possible)}. 
Nevertheless, \tool can be viewed as a transformation schema which automatically learns these patterns without human guidance. We note that \tool is \emph{not} explicitly focused on bug-fix changes since it is trained with generic changes. Even then, \tool achieves good performance in \defj bugs. Thus, we believe \tool has the potential to complement existing program repair tools by customizing the training with previous bug-fix patches and allowing to learn from larger change sizes. 
Given time and space limitations, we leave this to future work. 



%SequenceR considers 75 Defects4J bugs that have been fixed with a one-line patch by human developers. In total, SequenceR finds 2,321 patches for 58 of the 75 bugs. The main reason that they are unable to fix the remaining 17 bugs is due to fact that some bugs are not localized inside a method, which is a requirement for the fault localization step that SequenceR assumes as input. Out of 75 bugs, SequenceR successfully generated at least one patch for 58 bugs, 53 bugs have at least one compilable patch, 19 bugs have at least one patch that passed all the tests (i.e., are plausible) and 14 bugs are considered to be correctly fixed (semantically identical to the human-written patch).

% In a recent paper,  Saha~\etal~\cite{saha2017elixir} showed that they could fix 11.93\% Defects4J bugs (26 out of 218). 
% They had 8 pre-defined fix patterns and applied those patterns to fix the bugs. 
% Similar pattern based bug-fixing approaches are also proposed in the past~\cite{kim2013automatic}. 
% \tool can be viewed as a transformation schema which automatically learns these patterns without any human guidance. In fact, \tool can fix three bugs that are also fixed by Saha~\etal
% Additionally, \tool can generate 2 (Math-46, Math-49) more complete fixes and 1 (Lang-46) partial fixes. Thus, without any human guidance, \tool can complement state-of-the-art program repair tool's performance. 


% %One thing to note here, these types are automatically identified and generalized by \tool. 


% \tool successfully generated the fixes for 22 buggy ASTs corresponding to 10 bug ids. These are all concrete patches.
% Among 8 of those 10 bug ids, \tool generated fixes for all the buggy ASTs (\ie 10\% of the studied bugs). 
% For other two bug ids, \tool generated partial fixes.  

% \input{tables/d4j.tex}

% Table~\ref{tab:defj_res} further shows all the patches 
% that \tool can successfully generate. 
% For all the bugs marked in~\Greenul{green}, \tool successfully fixes all the underlying buggy methods. For example, Math-49 has 4 buggy methods, \tool fixes all the four. 
% For the bugs marked in~\blued{blue}, \tool fixes all the methods that are in scope. For example, for Lang-46, there are 6 methods to be patched, 4 of them are in \tool's scope, and \tool fixes them. 
% However, for other two bugs (marked in~\Orange{orange}), 
% \tool produces only partial fix. For example, in the cases of Time-26 and Lang-60, although all the methods are within scope, \tool could fix 6 out of 7 and 1 out of 2 methods respectively.  
% The `Patch Type' column further shows the type of change pattern for those patches.



% %In a recent paper, Elixir by Saha~\etal~\cite{saha2017elixir} reported 26 fixed bugs in Defects4j dataset. Although, they had 4 projects from Defects4j in their scope. They deployed 8 pre-defined pattern from transformation of the buggy-program. \tool can be viewed as a transformation schema which automatically learns the pattern. \tool can fix 2 (Math-46, Math-49) more bugs completely and 1(Lang-46) partially than Elixir. Thus \tool can be complementary to the existing program-repair tools. 



==> case_study.tex <==
Let us further investigate the cases where \tool could predict correct patches in original dataset and \sts could not. In our experiment, in 216 cases, \tool could generate correct patch in top 20 where \sts could not. We manually investigated those 216 patches and assigned a category of the patch considering the change type. Table~\ref{tab:patch_case_study} shows the categories and number of patches in each category. 

\begin{table}[!htpb]
    \scriptsize
    \centering
    \begin{tabular}{l|c}
        \toprule
            \textbf{Patch Category} & \# of correct patch by \tool  \\
            \midrule
            API Change & 10\\
            Bracket Change & 8\\
            Type related change & 24\\
            Expression change & 2\\
            Changes related to $final$ keyword & 77\\
            Method modifier change & 20\\
            Method parameter change & 45\\
            Statement change & 4\\
            Other (misc.) & 26\\
            \bottomrule
    \end{tabular}
    \caption{\textbf{\small{Performance  of  \tool suggesting abstract patches}}}
    \label{tab:patch_case_study}
\end{table}

==> problem_definition.tex <==
\section{Problem Definition}
\label{sec:problem-def}

==> revision-comments/major-revision-reviewers-comments.tex <==
\pagebreak
\newpage
\pagenumbering{Roman}
\renewcommand{\baselinestretch}{0.75}
\renewcommand*{\thesection}{\Alph{section}}
\nobalance
\section*{RESPONSE TO REVIEWERS}
\bigskip

\section*{Response to the Editor}

Comments to the Author: 
All three reviewers agree that the topic of the paper is useful. However, all reviewers raise major concerns too. These range from over claims to clarifying issues to questions about some of the results. R2 (and to some extent R3) also has concerns about a comparison with the past state of the art. I recommend that the authors try their best to perform some kind of comparison. I suggest the authors perform a major revision and address every comment by the reviewers and prepare a reply letter with the details of the changes made. 

\begin{response}
Thank you very much for your comments. We have taken all the reviews into careful consideration and we have changed the manuscript to reflect the feedback. We hope the new draft satisfies all the issues and concerns raised by the reviewers. 

To assist the reviewers in tracking all the changes we have incorporated in this version, we have annotated changes with \respto{X-XX} to correspond to reviewers’ concerns.
\end{response}

\vspace{5mm}
% \section*{Reviewer: 1 }
\section*{Response to Reviewer - 1 }

%Public Comments (these will be made available to the author) 

% \textbf{SUMMARY }
% The paper presents a novel approach, as well as an associated tool named CODIT, for learning code edits which relies on Tree-Based Neural Models. CODIT is designed as a two-steps encoder-decoder model. In the first step a tree2tree model dels the probability distribution of changes. The first step is performed by a Tree Translation Model which learns how to suggest structural changes in the form of AST modifications. In particular, the LSTM-based encoder takes as input a sequence of grammar rules, encodes them in a vector representation. Next, this vector is consumed by the decoder which generates the tree of the modified code expanding grammar rules. In the second step, a Token Generation Model conditioned both on the input code and the output of the Tree model, generate concrete code for the suggested structural change. This model is constrained by a mask to suggest tokens that are compatible with the type. The authors compare their approach against a seq2seq baseline and SequenceR on three datasets: code changes, pull requests, and bug repair. The results show that CODIT outperforms the baselines on all three datasets considered. 

% \textbf{COMMENTS: }
% The paper is extremely well written and easy to follow. Motivations are well described and design decisions are clearly articulated. I strongly believe that the combination of a Tree model, which focuses on structural changes, and a Token generation model, responsible for code concretization, can outperform other approaches. I completely agree with the intuition behind this approach. However, the paper has some critical issues in terms of claims, applicability, and evaluation that needs to be addressed before it is ready for publication. I recommend a Major Revision.
\begin{response}
We thank you for your detailed and constructive reviews. We have made several modifications, clarification and changes to our manuscript that addresses your reviews and concern. We hope this version or our manuscripts is better suitable for publication thanks to your meticulous reviews and feedback. To assist further review process, we have annotated the changes with \respto{1-XX}
\end{response}

\vspace{3mm}
\textbf{R1-1. Out-Of-Vocabulary tokens }
An inexperienced reader could very well believe, from reading the paper, that CODIT solves the problem of out-of-vocabulary tokens. This is not true and should be clarified in the revised version. If a token is not in the vocabulary, nor in the input code (i.e., the copy mechanism cannot copy it from the input), this token cannot be suggested by CODIT. That is, if a developer introduces a new token during an edit, and this token is novel in the codebase, CODIT cannot concretize the change. The copy mechanism itself cannot solve all the problems. This is also important to understand in comparison with previous approaches. 

\begin{response}
Thank you for pointing this out. We agree that our previous text was misleading. We also agree that ``Vocabulary Explosion'' still 
remains an open problem. We pointed out this fact explicitly in 
the paper for general readers. \citeresp{1-1}
\end{response}

\vspace{3mm}
\textbf{R1-2. Comparison with Tufano et al.}
I believe that the section 6.2 should be carefully revised. The authors appear to suggest that, since the previous approach works on an “abstract” dataset, they compare CODIT on a somewhat “enhanced” version of  Tufano’s work using the copy mechanism. Tufano’s approach first abstracts the code, then translates it, then concretizes it. In this abstract representation there are original tokens (idioms that are in the vocabulary) and the rest are replaced with IDs. Then, the abstract code is translated into another abstract code. Finally, the code is concretized by mapping back IDs with the original tokens. The last step of mapping back IDs with tokens is a “sort of” copy mechanism, where the IDs are replaced with tokens coming from the input code. By dropping the abstraction step, and simply using vanilla seq2seq + copy mechanism, is not clear that the authors are actually “enhancing” Tufano’s approach. As a matter of fact, the abstraction step could create a representation of the code where learning transformations is easier and more effective. Therefore, I suggest the authors to compare against the original approach. 

{\it Claim: }
“For example, they cannot predict many literals that do not appear in the original version of the code.” If the literals do not appear in the Vocabulary (they call it “idioms”) nor in the original version of the code, neither Tufano’s approach nor CODIT can generate that literal. This refer to the first point that, if the token is not in the vocabulary nor in the input code, copy mechanism cannot handle it. 

{\it Claim: }
“In this way, both CODIT and Seq2Seq handle the vocabulary explosion problem in same way and can be compared fairly.” 
This comparison could be “fair” towards seq2seq, but definitely not towards Tufano’s approach, since the authors are getting rid of a fundamental step in that approach, in the name of “fairness”. I suggest the authors to simply compare with the original approach. Moreover, the results in the paper “On Learning Meaningful Code Changes via Neural Machine Translation” claim 16-21\% accuracy on top-1 even considering bigger methods than those considered in this paper. 

\begin{response}
We apologize for the confusion here. We have revised our methodology in~\Cref{subsec:baseline}~\citeresp{1-2}. 
%, to reflect more accurate description of different baselines that we compared against in this version. 
In this version, we compared against both Seq2Seq + Copy Attn where input code is augmented with additional context (similar to SequenceR~\cite{chen2018sequencer}), and Tufano~\etal's~\cite{tufano2018nmt_bug_fix} model. While Tufano~\etal's model is very good at predicting abstract code (see \Cref{tab:tree_prediction} for results), it predicts a lot of abstract tokens that we are unable to concretize. 
For instance consider the following (dummy) scenario,\\

\noindent\textbf{Input Abstract Code :}
\vspace{3mm}
\begin{lstlisting}
public TYPE_1 METHOD_1(int VAR_1){ return VAR_1 * VAR_1; }
\end{lstlisting}
\vspace{3mm}
\noindent\textbf{Output Abstract Code:}
\vspace{3mm}
\begin{lstlisting}
public TYPE_1 METHOD_1(int VAR_1){ return VAR_1 * @\textbf{VAR\_2}@; }
\end{lstlisting}
\vspace{3mm}

Notice that, the output code contains an abstract identifier {\ie, \tt{VAR\_2}}, which cannot be concretized to the original form. 
While these examples are very informative for developers and could guide developers, in RQ1, we only considered examples which can be fully concretized~\citeresp{1-2}.
\end{response}

\vspace{3mm}
\textbf{R1-3. Granularity and Size }
While the extraction process starts at method granularity, the actual learning happens at fragment level (i.e. one/few lines of code). This means that at inference time, the developer needs to feed a particular fragment of code, not an entire method or class. Given the size thresholds used in the paper, these fragments appear to be quite small. Please, provide in the paper the distribution of \#tokens for these input/output fragments. 

\begin{response}
We have provided the statistics of the examples in the datasets we used in terms of number of tokens and number of tree nodes~\citeresp{1-3}.
\end{response}

\vspace{3mm}
\textbf{R1-4. Code and Tree Duplication }
Code duplication can artificially inflate the performance of ML approaches, as found by one of the authors in: “The Adverse Effects of Code Duplication in Machine Learning Models of Code”. In this paper, I did not find any mention of de-duplication efforts on the dataset used. Are there duplicate fragments pairs within the train/validation/test sets? What about the Tree/Grammar Rules representation of the code fragments? Are there duplicates in such a representation? I believe it’s fine to have duplicates in a high-level representation such as Tree/Grammar Rules, however, the authors should report the amount of duplicates in such a representation, in order to have a better idea of the prediction capabilities of the Tree Translation Model. For example, we could see that there are only very few patterns of tree transformations that dominate both train/test set. This means that the Tree Translation Model is simply repeating the same tree transformation found in the test set, also in the training set. 

\begin{response}
Thanks for pointing this out. Our previous version of the dataset had some duplication. These duplication include both intra-split and inter-split duplications. In the previous version of the dataset, we considered one commit only once and split the dataset based on project chronology, thus these duplications are indicative of the fact that developers re-use similar changes. 
%We leave investigation of those repetitive changes for other research. 
Nevertheless, in this version, we de-duplicated both intra and inter-split duplicates and reported the results in de-duplicated dataset~\citeresp{1-4}.
\end{response}

\vspace{3mm}
\textbf{R1-5. Clarification: Unfeasible Grammar Rules }
It’s hard for me to understand how the Tree Translation Model guarantees the generation of syntactically correct edits. The learning happens through learned vector representations and, especially when using beam search, some unfeasible grammar rules could potentially be selected during the translation. While the Token Generation Model uses a mask to make sure that only particular tokens are selected, I do not see any mask or mechanism to force the model to always select feasible grammar rules in the Tree Translation Model. Please, provide the intuition and details (and maybe references) on how this model guarantees the syntactic correctness of all the generated trees.

\begin{response}
In the beam search, while expanding a tree node, we consider the {\tt frontier\_node}($n_f^t$) at every time step, we ignore any CFG rule whose head does not match with $n_f^t$. This way, we ensure the syntactic correctness of the generated tree. Such strategy was also used by Yin~\etal~\cite{yin2017syntactic}~\citeresp{1-5}.
\end{response}

\vspace{3mm}
\textbf{R1-6. Clarification: Multiple scopes \& types }
How does the Token Generation Model deal with variables defined in multiple/different scopes? What about same variables names that are used for different types of variables? 

\begin{response}
If a variable is defined at a different scope and is not reachable from the change context, we consider that variable as out of scope. As for your second point, Java (or any strict typed language) does not support using same variable with different type(s) in the same scope. In weakly typed languages (\eg, Python, Javascript), this is possible. Since in this prototype version of \tool, we evaluated on Java projects, we do not explicitly consider a scenario where variables names that can be used for different types of variables.
% While in current version of \tool, we guarantee syntactic correctness, 
% ~\bray{I think he is asking about variable overloading, not type correcness} %type correctness of 
% variable overloading (same variable names used for different types in the same context) is out of \tool's scope. % and still remains an open problem.
\end{response}

\vspace{3mm}
\textbf{R1-7 Data \& Open Science}
In 2020, I would expect every research paper to publicly release data and code to allow reproducibility of the study. Would the authors commit to release the source code of CODIT? Personally, I believe that reviewers should have access to at least part of the data (input, outputs, representations of the fragments) so to perform a minimum of examination before acceptance. 

\begin{response}
% \bray{what about the data?}
 - We have released our prototype implementation at \url{https://github.com/saikat107/Codit}.
 
 - The dataset is available at \url{https://drive.google.com/file/d/1wSl_SN17tbATqlhNMO0O7sEkH9gqJ9Vr/}.
\end{response}

\vspace{3mm}
\textbf{R1-8 Typos }

Page 2: “model concertizes” $->$ “model concretizes” 

Page 5: “we to create a mask” 

\begin{response}
Thanks for the correction. We have corrected these. Our apologies for those. 
\end{response}


% \textbf{\#\# Strengths }

% + Potentially a superior approach with Tree + Token models; 

% + Large empirical analysis on different datasets; 

% + Very well written paper. 

% \textbf{\#\# Weaknesses }

% - Missing comparison with previous approach; 

% - CODIT works only on small fragments; 

% - Possible code duplication; 

% - No data/code released yet. 

% \begin{response}
% Thanks for the great review and help us make 
% \end{response}
% \balance
% \newpage
\vspace{3mm}
\section*{Response to Reviewer 2 }

\begin{response}
Thank you for your detailed and meticulous reviews and feedback. We have revised our manuscript based on your reviews, answered the clarification question that you had. We hope this version of the manuscript is suitable for publication. To assist further review process, we annotated the modifications based on your reviews with \respto{2-XX}.
\end{response}
% Public Comments (these will be made available to the author) 

% This paper proposes CODIT, a tree based neural model for suggesting source code changes. CODIT is given the previous version of source code, and predicts the changes. It uses a two step encoder-decoder model, with a tree translation model and a token generation model. The tree translation model predicts the AST level structure change. The token generation model then predicts the actual value of newly created nodes, which is dependent on the structure change predicted by the tree translation model. CODIT is evaluated on three tasks and datasets: 1) Code-Changes-Data is a dataset of commit history collected by the authors, the task is to predict the commit change. 2) Pull-Request-Data is dataset of pull request collected by previous research, the task is to predict the PR. 3) Bug-Repair-Data is a dataset of single-statement bug fixes, the task to fix single line bugs in Defects4J. Each task is compared against a seq2seq baseline or against previous research. The authors finds that CODIT outperforms the baseline and previous research on all three tasks. 


% \textbf{Strengths: }

% * Important problem: automating code changes to reduce the developers’ burden. 

% * Novel approach by dividing the code change prediction tasks into two phases: structure prediction and token prediction. 

% * Good evaluation: the evaluation of both the tree translation model and the token generation model is great. The authors use three different dataset and tasks, and showed improvements on all tasks. 

% \textbf{Weaknesses: }

\vspace{3mm}  
\textbf{R2-1. Scope of \defj bugs.} 

- The focus on the single-line bug on RQ3 is weird. Based on the description of CODIT, the model should be capable of generating more general bug fixes, even if it limited by the max\_change\_size and max\_tree\_size value. 

- The focus on the single-line bug on RQ3 is not justified. We would like to see the performance on all Defects4j bugs and not only one-liners. 

% \begin{response}
% Thank you for the suggestion. As we mentioned earlier, in this version, we have revised RQ3 to go beyond one line bugs.  
% \end{response}

\begin{response}
Thanks for pointing this out. We apologize for the confusion in RQ3.  We have revised RQ3, where we increased \tool's scope beyond 1 line bug fixes. We define the current scope of \defj bug fixes to be $max\_change\_size=10$ and $max\_tree\_size=20$~\citeresp{2-1}.
\end{response}

\vspace{3mm}
 \textbf{R2-2. Lack of Baselines and Discussion.} Lack of comparison against other techniques that also explicitly predict structure and token changes, such as [1] and [2] (see reference below). A quantitative comparison would strengthen the paper for publication. 

\begin{response}
Thanks for these suggestions. We have added a discussion detailing relevant research works including the ones you suggested~\citeresp{2-2a}. In our opinion, Brockschmidt~\etal~\cite{brockschmidt2018generative} technique addresses fundamentally different problem than ours. While their model focuses on generating expressions, which is vaguely similar to code completion. Tarlow~\etal~\cite{tarlow2019learning}'s work is very similar to us, and we believe it can augment \tool's approach. 
Unfortunately, their implementation is not publicly available. 


Nevertheless, to understand different types of encoder in \tool's pipeline, we compared against several other baselines \ie, Tree2Seq, Code2Seq~\citeresp{2-2b}. Note that both Tree2Seq and Code2Seq are tree based approaches.
% \bray{Copy the whole text in baseline as well.}
We also did some experiment on Kommrusch~\etal~\cite{kommrusch2020equivalence}'s proposed Graph2Seq network, which they provided implementation as an add on in OpenNMT-Py framework \url{https://opennmt.net/OpenNMT-py/ggnn.html}. However, their implementation is assumed upon a very restricted vocabulary size. To understand better, we modified their code to fit 
into our context, but neither their original model, nor our 
modified model works in program change task. When we increase the vocabulary size in their version of the model, it does not scale and quickly exhaust all the memory in the machine (we tried their model on a machine with 4 Nvidia TitanX GPU and 256 GB RAM). When we tested our modification of their code, the model does not converge even after 3 days of training, eventually resulting in 0 correct predictions~\citeresp{2-2c}. 


\end{response}

\vspace{3mm}
\textbf{R2-3. Lack of detailed ablation.}

* Some details, explanations of design choice and fixes values are missing. There are described in the comments below. 

* We need experimental results on the impact of the training data size on the model performance. 

* We need experimental results on the impact of parameters max\_change\_size and max\_tree\_size on the model performance. 

\begin{response}
Thanks for the suggestion. ``max\_change\_size'' and ``max\_tree\_size '' are two data collection hyper-parameters, which we used for collecting \dataname. In RQ2 of this version of the paper, we have shown the ablation study to show sensitivity of the these two parameters. As for the ablation on the training data, varying these two parameters ultimately results in different training data size~\citeresp{2-3}.
\end{response}

\vspace{3mm}
\textbf{R2-4. Scalability of the model }
One concern is the scalability of the model. For larger code changes, the AST will contain much more production rules and any wrongly predicted production rule will lead to uncompilable / meaningless code edits. 

\begin{response}
Thanks for pointing out this fact. We agree with the fact that larger AST contains many productions rules. However, being a tree based model, \tool can guarantee syntactic correctness. We agree that semantic correctness still remains an open problem. In any case, our endeavor  in \tool to focus on automating the smaller changes, so that developers can focus on more complex changes. For larger changes, we envision a developer assistance tool, which we leave for future research.
\end{response}


\vspace{3mm}
\textbf{R2-5. Dataset and Code }
The replication package for the paper is not available. In particular, the authors claim "a large dataset of 44k real code changes" as one of the three key contributions, but the dataset is not accessible.

\begin{response}
- Our prototype implementation is available at \url{https://github.com/saikat107/Codit}. 

- The dataset is available at \url{https://drive.google.com/file/d/1wSl_SN17tbATqlhNMO0O7sEkH9gqJ9Vr/}.
% \bray{where is the dataset?}
\end{response}



% The focus on the single-line bug on RQ3 is not justified. We would like to see the performance on all Defects4j bugs and not only one-liners. 

% \begin{response}
% Thank you for the suggestion. We apologize for the confusion in RQ3. As we mentioned earlier, in this version, we have revised RQ3 to go beyond one line bugs.  
% \end{response}

% A discussion comparing your approach and probabilistic context-free grammar s(‘ref above) is needed. 

% \begin{response}
% Thanks for pointing this out. We have added a discussion summarizing the recent works in grammar based code modeling, and structure based code modeling~\citeresp{2-3}. 
% \end{response}

\vspace{3mm}
\textbf{R2-6. Clarification on \tool's architecture and working procedure}

 - Sentences between line 45-50 at page 4 where you describe the mask. Does it mean CODIT cannot generate new type, method and variable name? 


 - You mentioned that you used the copy mechanism in CODIT. But you only describe it between line 52-55 at page 4. It is not clear if what you have described is the copy attention, or the process after the copy mechanism has failed. 
 
 - In section 6, it is not clear if you used the same max\_change\_size and max\_tree\_size for all datasets, 


\begin{response}
Thanks for pointing out this important fact. With the mask, we let the \tokenmodel choose appropriate tokens given a {\tt frontier\_node} type. When the node type is variable, method name and type name, we restrict \tokenmodel's choice between allowed tokens (which we extract based on the variable reachability in pre-processing step). We also provide the special {\tt <unknown>} token as another option to \tokenmodel. In the case, when \tokenmodel predicts {\tt <unknown>}, we replace that {\tt <unknown>} with the source token with highest attention probability. Note that, \tool is not trained to copy tokens, \ie, in training phase, there is no copy. The copy mechanism takes place during the beam search and only to prevent the prediction of {\tt <unknown>} token. Nevertheless, we agree with you that \tool cannot generate new type, method and variable name. \tool can choose between the tokens that are in the vocabulary or in the input code. We have modified the manuscript to remove these confusions~\citeresp{2-6}. As for your third point, in this version of the manuscript, we set the same limit for those two parameters across all datasets. 
\end{response}

% \begin{response}
% Thanks for pointing out this fact. 
% \end{response}

\vspace{3mm}
\textbf{R2-7. Clarification on data statistics} In section 6, I wish to see the number of method pairs before and after applying max\_change\_size and max\_tree\_size filter. For Code-Change-Data, you only described that you had 241,976 file pairs and 44,382 method pairs after. For Pull-Request-Data and Bug-Repair-Data, it is not clear if the number of method pairs are before or after filtering. By giving this number it will also give us an idea how general the approach is. 

\begin{response}
While in \dataname, we collected example with max\_change\_size = 10 and max\_tree\_size = 20, we found 182,952 method pair before applying these filter, while after applying these filters we get 44,382 patches~\citeresp{2-7a}.  As for \icsedata, we get 5,546 examples out of 21,774 after applying the same filter~\citeresp{2-7b}.  
\end{response}

\vspace{3mm}
\textbf{R2-8. Correction on mis-representaion.}
 The section ‘Evaluating tree translation model’ between page 7 and 8, I believe all M\_{token} should be M\_{tree} since you are describing the how M change the tree structure. 

\begin{response}
Thanks for pointing our this. We apologize for this confusion. You are right, those will be \treemodel. In this version, we have corrected those~\citeresp{2-8}.
\end{response}

\vspace{3mm}
\textbf{R2-9. Clarification on ablation result.}
In table 8, we see a decrease of performance when increasing the beam size K\_{tree}. Usually, increasing the beam size always increase the performance, for example see table III in [5]. What’s the explanation for this? 

\begin{response}
It is true, with the increasing number of beam size, the performance increases. which is also evident in results that we presented in~\Cref{tab:concrete}. However, the ablation we showed in \Cref{tab:k1k2} is not directly an ablation of tree beam size. Rather, it is an ablation of how many trees that \tool considers for expanding. For examples, when \ktoken is 10 and \tool is considering 2 trees (\ie, \ktree = 2), \tool generates 20 code, among which \tool chooses top 10 code based on \cref{eqn:mainprob}. With increasing value of \ktree, \tool faces with more options to choose from which ultimately hurts \tool's performance~\citeresp{2-9}.
\end{response}

% References: 

% [1] Brockschmidt, Marc, et al. "Generative code modeling with graphs." arXiv preprint arXiv:1805.08490 (2018) 

% [2] Tarlow, Daniel, et al. "Learning to Fix Build Errors with Graph2Diff Neural Networks." arXiv preprint arXiv:1911.01205 (2019) 

% [3] Chen, Zimin, et al. "Sequencer: Sequence-to-sequence learning for end-to-end program repair." IEEE Transactions on Software Engineering (2019). 

% [4] Cho, Kyunghyun, et al. "On the properties of neural machine translation: Encoder-decoder approaches." arXiv preprint arXiv:1409.1259 (2014). 

% [5] Tufano, Michele, et al. "On learning meaningful code changes via neural machine translation." Proceedings of the 41st International Conference on Software Engineering. IEEE Press, 2019. 

% \balance
% \newpage
\vspace{3mm}
\section*{Response to Reviewer 3}

% 
\begin{response}
We appreciate your thoughtful review and feedback on our manuscript. We made enhancement, corrections to our manuscript based on your feedback. We hope this version of the macnuscript is better suitable for publication. To assist further review process, we annotated the manuscript with \respto{3-XX} where we made changes based on your feedback. 
\end{response}

\vspace{3mm}
\textbf{R3-1. The Definition of code change and the changing scope concerned in this paper.} 

1. The term “code change” is vaguely described across the paper, I would recommend authors to give a brief formal definition of what “code change” exactly means in this paper. 

2.  In addition, it might be better if the change level or scope could be clearly described at an early stage of the paper, for example, on the whole software project level, file level, class level, or method level. It is not until I reach the later part, I found that the paper is actually focusing more on the method level. 

 Again, I would recommend to clearly define what the “small” code change means, and be clear about the potentially applicable scope of the technique.

\begin{response}
We thank you for bringing out this point. We apologize for not being clear upfront in the previous version. To answer to your first point, following previous researches~\cite{ying2004predicting, zimmermann2005mining, kim2007automatic, tufano2019learning}, we define automatic ``code change'' as modification or editing of code with frequent change patterns~\citeresp{3-1a}. 
As for your second question, in theory, \tool can be used in any small code fragment of any programming language. However, for prototyping and proof-of-concept test, we designed \tool to learn changes that belong to methods in java classes~\citeresp{3-1b}.
\end{response}

\vspace{3mm}

\textbf{R3-2. The code changing patch data collection }
·  Changing patch data collection is an important contribution of this paper. I highly appreciate the authors’ effort. However, the authors only give a very brief summary of the statistics of this data. I would recommend giving more detailed information on how the data is collected, and how they are preprocessed until reaching the state that is ready for further training. For example, how the project repositories are selected, what scientific rules and procedure are followed? Are the selected repository representative that cover a wide range or type of applications? 
·  In addition, I would also recommend adding more statistical information about the collected data for training. For example, what is the changing size in terms of code lines for these batch? This might be relevant to what kind of changes the model might be able to handle or generalize. 

\begin{response}
For \tool prototype, we choose Java projects from TravisTorrent~\cite{msr17challenge} challenge which is used in MSR mining challenge 2017. All the projects in that datataset are non-forked, non-toy project with somewhat popularity ($>$ 10 watchers in guthub). On top of that, those projects are well maintained and big enough projects. While there is no pre-defined measure of how well maintained a project repository in github is, all the projects in TravisTorrent dataset uses Travis Continuous Integration, which gives us an intuition that those are well maintained (otherwise CI would fail frequently causing the developers a lot of overhead). 
%In a repository, there are a lot of 
Further, we only selected projects with at least 50 commits in master branch that changes at least one java files, which indicates that those projects actively go through a lot of source code changes. In this version of the manuscript, we have revised the \Cref{sec:experiment} and included these details~\citeresp{3-2}. As we have shown in ~\Cref{examples}, \dataname contains a wide variety example types. As for your second suggestion, we added statistical information of the dataset in \Cref{tab:dataset_summary}. 
\end{response}

\vspace{3mm}
\textbf{R3-3. The evaluation }

1. For RQ 1, from my point of view,  evaluating the generalization of the model is very important. Therefore, it would be important to see whether the model trained on a project set A could be generalized to project set B, where A and B do not overlap. 

2. For the detailed training and evaluation, I am not exactly sure how the training data are used for training the model (please correct if I miss in the paper). Whether splits among projects are considered instead of patches. 

\begin{response}
Thanks for suggesting this experiment. We have conducted this experiment to check \tool's capability of cross-project generalization\citeresp{3-3a}. Our experimental results show while full-\tool performs worse in cross-project evaluation setting than our current intra-project splits, the \treemodel (structure transformation model) performs equally well in intra-project and cross projects setting. We conjecture that, a wide range of project specific identifiers is the main reason of such degradation. Also we found an interesting finding that structural changes in code are more ubiquitous across different projects. 
\end{response}

\begin{response}
As for your second question, to mimic the real world development scenario, we divided the dataset into train, validation and test split based on the chronology of the changes --\ie, first 70\% commits in each project's timeline goes to train set, next 10\% to validation set, rest 20\% to test set~\citeresp{3-3b}. On top of that, we de-duplicate any intra-split and inter-split repetitions.
\end{response}

\vspace{3mm}
\textbf{R3-4. Relevant baseline. }
For RQ 2, I appreciate the authors’ effort in design choice study. Here, The code2seq would be a highly relevant paper. Although the application scenario is a bit different, it should be easily adapted to change recommendations as well. I understand the comparisons might be difficult, at least some discussion should be made to stress the similarity and difference. Code2seq: Generating Sequences from Structured Representations of Code, ICLR 2019 

\begin{response}
Thank you for the suggestion. We agree that Code2Seq is a highly relevant baseline. We have compared with code2seq for code change task in~\Cref{sec:experiment} (see~\Cref{tab:concrete} for results). One important aspect that we noticed is that, while the stochastic nature of input code representation in code2seq is helpful for natural language generation (original use case for Code2Seq), that same stochasticity actually confused the attention mechanism in code generation~\citeresp{3-4}. Saying that, we have tried Code2Seq as is for the code change task, and we believe some modification in Code2Seq architecture might augment \tool's performance. Such modifications, however, are beyond the scope of this research.
% \bray{mentions the table to look at for code2seq result.}
\end{response}

\vspace{3mm}
\textbf{R3-5. Experimental setting of RQ3.} For RQ 3, although one line fixing results shows to be promising. I would recommend also include other bugs beyond one line and see how the technique works. From my perspective, demonstrating the capability of the techniques is definitely important, showing and discussing its limitation is important as well, e.g., giving typical examples where the technique fails to work. 

\begin{response}
Thanks for the suggestion. We have revised RQ3 to incorporate bugs beyond 1 line bugs~\citeresp{3-5a}.
As for your second point, we appriciate your suggestion. We have added a discussion of limitation of current \tool in program repair settings~\citeresp{3-5b}. One cruicial limitation right now is, \tool does not consider interaction between different hunks in a multi-hunk bug. We leave such investigation as future work. 
\end{response}

% In summary, this paper works on an important topic. The proposed techniques are also quite promising. I hope the authors would consider the aftermentioned issues during revision before publication.

==> tables/abs_res.tex <==
% Table generated by Excel2LaTeX from sheet 'summary_result'
\begin{table*}[htbp]
\scriptsize
\setlength{\tabcolsep}{2pt}
  \centering
  \caption{\textbf{\small{Performance of \tool suggesting abstract edits ~\sk{Is it MAP?}
  %Number of correctly generated patches in top 1/2/5/10/20 patches are shown in the table. In each case, performance of \tool with copy, without copy and also performance of a sequence-2-sequence model are shown.
  }}}
    %\begin{tabular}{|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc}
    \toprule
      &  & 
    \multicolumn{3}{c|}{Top 1} & 
    \multicolumn{3}{c|}{Top 2} & 
    \multicolumn{3}{c|}{Top 5} &
    \multicolumn{3}{c|}{Top 10} &
    \multicolumn{3}{c}{Top 20} \\
            \cline{3-17}
    \textbf{Edit} &  &  \multicolumn{2}{c}{\tool}  &  &  \multicolumn{2}{c}{\tool}   &   &  \multicolumn{2}{c}{\tool}   &   & \multicolumn{2}{c}{\tool}   &   &  \multicolumn{2}{c}{\tool}   &  \\ \cline{3-4,6-7,9-10,12-13,15-16}
    \textbf{Sizes} & \textbf{\#Examples} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} \\
    \midrule
    1     & 3368  & 586   & 33    & 299   & 785   & 36    & 330   & 1043  & 37    & 460   & 1208  & 41    & 704   & 1358  & 65    & 818 \\
    %\midrule
    2 - 5 & 2061  & 22    & 7     & 1     & 59    & 14    & 3     & 119   & 17    & 27    & 168   & 19    & 39    & 227   & 29    & 87 \\
    %\midrule
    6 - 10 & 1306  & 0     & 2     & 0     & 135   & 164   & 0     & 178   & 166   & 0     & 191   & 166   & 0     & 202   & 168   & 2 \\
    %\midrule
    %11 - 15 & 96    & 0     & 0     & 0     & 1     & 1     & 0     & 1     & 2     & 0     & 1     & 2     & 0     & 1     & 2     & 2 \\
    \midrule
    % Total & 6831  & 608   & 42    & 300   & 979   & 214   & 333   & 1340  & 220   & 487   & 1567  & 226   & 743   & 1787  & 262   & 909 \\
    % \bottomrule
    
   {Total} & {6735} & {608} & {42} & {300} & {979} & {214} & {333} & {1340} & {220} & {487} & {1567} & {226} & {743} & {1787} & {262} & {907} \\
          &       & 9.00\%  & 0.62\%  & 4.44\%  & 14.50\% & 3.17\%  & 4.93\%  & 19.84\% & 3.26\%  & 7.21\%  & 23.20\% & 3.35\%  & 11.00\% & 26.46\% & 3.88\%  & 13.43\% \\
   \bottomrule
    \end{tabular}%
    
  \label{tab:abs_res}%
\end{table*}%


==> tables/abstract.tex <==
% Table generated by Excel2LaTeX from sheet 'summary_result_paper'
\begin{table*}[htbp]
%\setlength{\tabcolsep}{1pt}
%\renewcommand*{\arraystretch}{1}
  \centering
  \scriptsize
  \caption{\textbf{\small{Performance  of  \tool suggesting abstract patches}}\vspace{-10pt}}
    \begin{tabular}{c|c|cc|cc|cc|cc|cc}
    \toprule
    Edit &       & \multicolumn{2}{c|}{Top 1} & \multicolumn{2}{c|}{Top 2} & \multicolumn{2}{c|}{Top 5} & \multicolumn{2}{c|}{Top 10} & \multicolumn{2}{c}{Top 20} \\
    {Sizes} & {\#Examples} & {CODIT} & {Seq2Seq} & {CODIT} & {Seq2Seq} & {CODIT} & {Seq2Seq} & {CODIT} & {Seq2Seq} & {CODIT} & {Seq2Seq} \\
    \midrule
    {1} & {3368} & {586} & {299} & {785} & {330} & {1043} & {460} & {1208} & {704} & {1358} & {818} \\
    {2 - 5} & {2061} & {22} & {1} & {59} & {3} & {119} & {27} & {168} & {39} & {227} & {87} \\
    {6 - 10} & {1306} & {0} & {0} & {135} & {0} & {178} & {0} & {191} & {0} & {202} & {2} \\
    \midrule
    {Total} & {6735} & {608} & {300} & {979} & {333} & {1340} & {487} & {1567} & {743} & {1787} & {907} \\ 
       &       & 9.03\%  & 4.45\%  & 14.54\% & 4.94\%  & 19.90\%  & 7.23\%  & 23.27\% & 11.03\% & 26.53\% & 13.47\% \\ \midrule
     \multicolumn{2}{l|}{Gain $(\frac{CODIT-Seq2Seq}{Seq2Seq})$}   & \multicolumn{2}{c|}{102.92\%} & \multicolumn{2}{c|}{194.33\%} & \multicolumn{2}{c|}{175.24\%} & \multicolumn{2}{c|}{110.97\%} & \multicolumn{2}{c}{96.96\%} \\
    \bottomrule
    \end{tabular}%
  \label{tab:abstract}%
\end{table*}

==> tables/abstract_examples.tex <==
%!Tex root=../main.tex


% \begin{table*}[!htbp]
% \scriptsize
%     \centering
%     \begin{tabular}{r|p{0.23\textwidth}|p{0.23\textwidth}|p{0.23\textwidth}|c|c}
%         \toprule
%         & & & & \multicolumn{2}{c}{Correct}\\
%         \cline{5-6}
%         Sl. & {\tt source} code $S$ &  {\tt target} code generated by \tool & {\tt target} code by \seq &  & \\
%         \midrule
%         1 &
%         \lstinputlisting[ language=java]{abs_examples/ex_1_parent.java}
%         & 
%         \lstinputlisting[ language=java]{abs_examples/ex_1_child.java}
%         &
%         \lstinputlisting[ language=java]{abs_examples/ex_1_seq.java} & Y & N
%         \\
%         \\
%         \midrule
%         2 &
%         \lstinputlisting[ language=java]{abs_examples/ex_2_p.java}
%         & 
%         \lstinputlisting[ language=java]{abs_examples/ex_2_c.java}
%         &
%         \lstinputlisting[ language=java]{abs_examples/ex_2_s.java} &Y &N
%         \\
%         \\
%         \midrule
%         3 &
%         \lstinputlisting[ language=java]{abs_examples/ex_3_p.java}
%         & 
%         \lstinputlisting[ language=java]{abs_examples/ex_3_c.java}
%         &
%         \lstinputlisting[ language=java]{abs_examples/ex_3_s.java} &Y &Y
%         \\
%         \\
%         \midrule
%         4 &
%         \lstinputlisting[ language=java]{abs_examples/ex_4_p.java}
%         & 
%         \lstinputlisting[ language=java]{abs_examples/ex_4_c.java}
%         &
%         \lstinputlisting[ language=java]{abs_examples/ex_4_s.java} &Y &Y
%         \\
%         \\
%         \midrule
        
%     \end{tabular}
%     \caption{\textbf{\small{Changes generated by tree2tree vs.~seq2seq model}}}
%     \label{tab:examples}
% \end{table*}

\begin{table}
\centering
\small
\begin{tabular}{l}
\toprule
\textbf{Ex1.~Correctly suggested by \tool but not by \sts} \\ \midrule
\begin{lstlisting}%[enhanced]{Correctly created by t2t but not by s2s}

src: public t3 () { t2 (); t4 . t1 (STR);} 
tar: public t3 () { t2 (); @\Red{\sout{t4 . t1 (STR);}}@ }

t2t: public t3 () { t2 (); @\Red{\sout{t4 . t1 (STR);}}@ } @\cmark @
s2s: public bool t3 () { t1 . t2 (STR) ;} @~~\xmark @
\end{lstlisting} \\
\\ \midrule\midrule
\textbf{Ex2.~Correctly suggested by both \tool and \sts} \\ \midrule
\begin{lstlisting}%[enhanced]{Correctly created by both}

src: private t1 () {}
tar: private t1 () {@\Green{super()}@;}

t2t: private t1 () {@\Green{super()}@;} @\cmark @
s2s: private t1 () {@\Green{super()}@;} @\cmark @
\end{lstlisting} \\ 
\\ \midrule\midrule
\textbf{Ex3.~Correctly suggested by \sts but not by \tool} \\ \midrule
\begin{lstlisting}%[enhanced]{s2s yes, t2t no}

src: { return new t2 ( new t1 ( null , true ) ) ; }
tar: { return new @\Red{\sout{t1 ( null , true ) )}}@  @\Green{t3 ()}@ ; }

t2t: { return new @\Red{\sout{t1 ( null , true ) )}}@  @\Green{t2 ()}@ ; } @\xmark @
s2s: { return new @\Red{\sout{t1 ( null , true ) )}}@  @\Green{t3 ()}@ ; } @\cmark @
\end{lstlisting} \\ 
\\
\bottomrule
\end{tabular}
\caption{\textbf{\small{Example Patches generated by tree2tree vs.~seq2seq model}}\vspace{-10pt}}
    \label{tab:examples}
\end{table}



==> tables/api_examples.tex <==
\begin{table}[!htpb]
\centering
\small
\begin{tabular}{p{.90\columnwidth}}
\toprule
\begin{lstlisting}
return (DateOnly) instant.@\Red{\sout{toCopy}} \Green{\underline{withMillis}}@(iField.roundHalfEven(instant.getMillis()));
\end{lstlisting}\\
\midrule
\begin{lstlisting}
return instant.@\Red{\sout{toCopy}} \Green{\underline{withMillis}}@(addTo(instant.getMillis(), scalar));
\end{lstlisting}\\
\midrule
\begin{lstlisting}
return (DateTime) instant.@\Red{\sout{toCopy}} \Green{\underline{withMillis}}@(iField.add(instant.getMillis(), value));
\end{lstlisting}\\
\midrule
\begin{lstlisting}
return (DateOnly) instant.@\Red{\sout{toCopy}} \Green{\underline{withMillis}}@ (iField.set(instant.getMillis(), value));
\end{lstlisting} \\
%\\
\bottomrule
\end{tabular}
\caption{\textbf{\small{Example of API changes suggested by \tool}}}
\label{tab:example_api_change}
\end{table}

in ~\Cref{tab:example_api_change} shows few examples of API changes. In each of the examples, {\tt instant.toCopy( ... )} method call is replaced by {\tt instant.withMillis( ... )}.

==> tables/case_study.tex <==
\begin{table}[!htpb]
    \scriptsize
    \centering
    \begin{tabular}{l|c}
        \toprule
            \textbf{Patch Category} & \# of correct patch by \tool  \\
            \midrule
            Changes related to $final$ keyword & 77\\
            Method parameter change & 45\\
            Type related change & 24\\
            Method modifier change & 20\\
            API Change & 10\\
            Bracket Change & 8\\
            Expression change & 2\\
            Statement change & 4\\
            Other (misc.) & 26\\
            \bottomrule
    \end{tabular}
    \caption{\textbf{\small{Performance  of  \tool suggesting patches}}\vspace{-10pt}}
    \label{tab:patch_case_study}
\end{table}

==> tables/d4j.tex <==
\begin{table}[!htpb]
    \scriptsize
    %\setlength{\tabcolsep}{1pt}
    \begin{center}{
    \begin{tabular}{@{}lrr@{}}
    \toprule
    Project & BugId  & Patch Type \\ 
     \midrule
     \multirow{3}{*}{Chart} &  1 &  Condition Change\\
                            & 9 &  Insert Conditional Statement\\
                            & 11 &  Invocation from different variable.\\
    \midrule
     \multirow{6}{*}{Closure} &  65 &   Method Parameter Change\\
                        &  73 &   Method Parameter Change\\
                        & 86 &  Boolean Value Change\\
                        & 92 &   Api Change\\
                        & 93 &  Api Change\\
                        & 104 &  Condition Change\\
     \midrule
     \multirow{3}{*}{Lang} &  16 &  Insert Conditional Statement\\
                            & 24 &  Insert Conditional Statement\\
                            & 59 &  Method Parameter Change\\
     \midrule
     \multirow{7}{*}{Math} &   5 &   Return-Value-Change\\
                        &  33 &   Method Parameter Change\\
                        & 57 &  Data Type Change\\
                        & 70 &   Insert Method Parameter\\
                        & 75 &  Change Method Call\\
                        & 82 &  Condition Change\\
                        & 85 &  Condition Change\\
     \midrule
     \multirow{1}{*}{Time} &   19 &   Condition Change\\
     \bottomrule
    \end{tabular}
    \vspace{-0.5cm}
    \caption{\small{\textbf{\tool's performance on fixing Defects4J~\cite{just2014defects4j} bugs\vspace{-10pt}}}}
    \label{tab:defj_res}
    }\end{center}
    
    % \begin{flushleft}
    % {\scriptsize Green} rows are bug ids where \tool can produce complete patch. 
    %  Blue} rows are where \tool can fix all the methods that are in \tool's scope. 
    % \Orange{Orange} rows are where \tool could not fix all that are in \tool's scope.
    % % \vspace{-9mm}
    % }
    % \end{flushleft}
\end{table}

% \begin{table}[!htpb]
%     \scriptsize
%     \setlength{\tabcolsep}{1pt}
%     \begin{center}{
%     \begin{tabular}{c|c|c|c|c|r}
%     \toprule
%     Project & BugId & \#methods & \#methods  & \#methods  & Patch \\ 
%      & & to be  & in  & \tool  & Type\\
%      & & patched & scope & can fix \\
%      \midrule
%      \multirow{4}{*}{Chart &  8 &  1 &  1 &  1 &  Api Change\\
%                                       & 10 &  1 &  1 &  1 &  Method-Invocation\\
%                                       & 11 &  1 &  1 &  1 &  Variable-Name-Change\\
%                                       & 12 &  1 &  1 &  1 &  Api-Change\\
%     \midrule
%      \multirow{5}{*}{Closure &   3 &   2 &   1 &   1 &   Method-Invocation\\
%                                       &  75 &   2 &   1 &   1 &   Return-Value-Change\\
%                                       & 86 &  1 &  1 &  1 &  Boolean-Value-Change\\
%                                       & 92 &  1 &  1 &  1 &   Api-Change\\
%                                       & 93 &  1 &  1 &  1 &  Api-Change\\
%      \midrule
%      \multirow{5}{*}{Lang &   4 &   2 &   1 &   1 &   Method-Invocation\\
%                                   & 6 &  1 &  1 &  1 &  Method-Parameter-Change\\
%                                   & 21 &  1 &  1 &  1 &  Method-Parameter-Change\\
%                                   & 26 &  1 &  1 &  1 &  Method-Parameter-Add\\
%                                   &  30 &   5 &   1 &   1 &   Type-Change\\
%      \midrule
%      \multirow{8}{*}{Math &   6 &   13 &   1 &   1 &   Method-Parameter-Change\\
%                                   & 30 &  1 &  1 &  1 &  Type-Change\\
%                                   & \Orange{46 &  \Orange{2 &  \Orange{2 &  \Orange{1 &  \Orange{Ternary-Statement-Change\\
%                                   & 49 &  4 &  4 &  4 &  Object-Reference-Change\\
%                                   & 57 &  1 &  1 &  1 &  Type-Change\\
%                                   & 59 &  1 &  1 &  1 &  Ternary-Statement-Change\\
%                                   & 70 &  1 &  1 &  1 &  Method-Parameter-Add\\
%                                   & 98 &  2 &  2 &  2 &  Array-Size-Change\\
%      \midrule
%      \multirow{3}{*}{Mockito &  \Orange{6 &  \Orange{20 &  \Orange{20 &  \Orange{2 &  \Orange{Api-Change\\
%                                       &  25 &   6 &   1 &   1 &   Method-Parameter-Add\\
%                                       &  30 &   2 &   1 &   1 &   Method-Parameter-Add\\
%      \bottomrule
%     \end{tabular}
%     % \vspace{-1cm}
%     \caption{\small{\textbf{\tool's performance on fixing Defects4J~\cite{just2014defects4j} bugs.\vspace{-10pt}}}}
%     \label{tab:defj_res}
%     }\end{center}
    
%     \begin{flushleft}
%     {\scriptsize Green} rows are bug ids where \tool can produce complete patch. 
%      Blue} rows are where \tool can fix all the methods that are in \tool's scope. 
%     \Orange{Orange} rows are where \tool could not fix all that are in \tool's scope.
%     % \vspace{-9mm}
%     }
%     \end{flushleft}
% \end{table}

==> tables/design-choices.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/equation.tex <==
% \begin{table} 
% \centering 
% \scriptsize
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{l|l}
% \toprule
%  $\begin{array} {lcl} f(x) & = & (a+b)^2 \\ & = & a^2+2ab+b^2 \end{array}$ & c\\ 
% \hline 
%  $\begin{array} {r@{}l@{}} f(x) & {}= (a+b)^2 \\ & {}= a^2+2ab+b^2 \end{array}$ & f\\    \hline 
%  $\begin{aligned} f(x) & = (a+b)^2 \\ & = a^2+2ab+b^2 \end{aligned}$ &h \\ \hline 
% \end{tabular}
% \label{tab:eq}
% \end{table}

\begin{table*}[ht]
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\tabcolsep}{2pt}
\renewcommand*{\arraystretch}{0.1}
%\scriptsize
\small
\caption{\textbf{\small{Intermediate computations used in  Decoding. Model parameters $\mathbf{E_R}$, $\mathbf{W_R}$, $\mathbf{E_V}$, and $\mathbf{b_R}$ 
are optimized during training.
\vspace{-15pt}}}}
\label{tab:eq}
\centering

\begin{tabular}{l|l|c}
\toprule
\multicolumn{2}{c|}{\textbf{Task}} & \textbf{Computation} \\
\toprule
%===========================================================================
\multicolumn{2}{l|}{Generating hidden state $s'_t$ using LSTM at time $t$} 
&
\parbox{0.6\columnwidth}{
\begin{equation}
    \label{eqn:decode-h-update}
    s'_t = f_{LSTM}([a_{t-1},a_{p_t}, s'_{p_t}, n_f^t, c_t], s'_{t-1})
\end{equation}
}
\\ \midrule
%================================== Grammar Rule ===============================
\multirow{2}{*}{\parbox{2.5cm}{Probabilities\\ related to\\ Grammar rules}} 
& ApplyRule($r$) at time $t$ 
&
\parbox{0.6\columnwidth}{
\begin{equation}
\label{eqn:rule-prob}
%\scriptstyle
p(r|S,a_1...a_{t-1},n_f^t)=softmax((E_R \cdot (W_R s'_t+b_R) \cdot mask_r(n_f^t))
\end{equation}
}
\\ \cmidrule{2-3}
&
InsertToken($v$) at time $t$
&
\parbox{0.6\columnwidth}{
\begin{equation}
%\scriptstyle
\label{eqn:vocab-prob}
%p(v|S,a_1...a_{t-1},n_f^t)=softmax((E_V \cdot (W_V \cdot s'_t + b_V)mask_t(n_f^t))
p(v|S,a_1...a_{t-1},n_f^t)=softmax(E_V \cdot (W_V \cdot s'_t + b_V ))
\end{equation}
}\\ \midrule
%================================== Copy Mechanism ==============================
\multirow{2}{*}{\parbox{2.5cm}{Probabilities\\ related to\\ Copy }} 
& Copying from input
&
\parbox{0.6\columnwidth}{
\begin{equation}
    \label{eqn:ptr-net}
    p(w_i|copy,x,a_1a_2...a_{t-1}) = \frac{exp(\omega(h_i, [s'_t, c_t]))}{\sum_{j=1}^{j=n} exp(\omega(h_j, [s'_t, c_t]))}
\end{equation}
}
\\ \cmidrule{2-3}
&
Decision of copying
&
\parbox{0.6\columnwidth}{
\begin{equation}
    \label{eqn:copy-prob}
    p(copy_t|S, a_1...a_{t-1}) = softmax(W_C \cdot s'_t)
\end{equation}
}\\ 
\bottomrule
\end{tabular}
\end{table*}

% \begin{multline}
%     \label{eqn:vocab-prob}
%     p(v|x, a_1...a_{t-1}, n_f^t) =  softmax((E_V \\
%         (W_V  s_t + b_V )  mask_t(n_f^t))
% \end{multline}

==> tables/gold-tree-vs-s2s.tex <==
\begin{table}[!htb]
    \scriptsize
    \centering
    \caption{\textbf{\small Correct patches generated by the standalone token generation model when the true tree structure is known.
    \vspace{-2mm}}}
    \label{tab:gold_tree}
    %\setlength{\tabcolsep}{2.5pt}
%\renewcommand*{\arraystretch}{1}
    \begin{tabular}{c|c|c}
        \toprule
         \multirow{2}{*}{Dataset} &\multicolumn{2}{c}{ Total Correct Patches}\\
         
          & \sts & standalone \tokenmodel \\
         \midrule
         \dataname & 545 (7.97\%) & 1509 (22.09\%)\\
         \icsedata & 73 (6.89\%) & 250 (23.63\%)\\
         \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}


==> tables/org_res.tex <==
% Table generated by Excel2LaTeX from sheet 'Summary_res'
% Table generated by Excel2LaTeX from sheet 'Summary_paper'
\begin{table*}[htbp]
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \centering
  \caption{\textbf{\small{Performance of \tool suggesting concrete edits
  %Number of correctly generated patches in top 1/2/5/10/20 patches are shown in the table. In each case, performance of \tool with copy, without copy and also performance of a sequence-2-sequence model are shown.
  }}}
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc}
    \toprule
          &       & \multicolumn{3}{c}{{Top 1}} & \multicolumn{3}{c}{{Top 2}} & 
          \multicolumn{3}{c}{{Top 5}} & 
          \multicolumn{3}{c}{{Top 10}} & 
          \multicolumn{3}{c}{{Top 20}} \\
    \cline{3-17}
    \textbf{Edit} &       & \multicolumn{2}{c}{\tool} &       & \multicolumn{2}{c}{\tool} &       & \multicolumn{2}{c}{\tool} &       & \multicolumn{2}{c}{\tool} &       & \multicolumn{2}{c}{\tool} &  \\ \cline{3-4,6-7,9-10,12-13,15-16}
    \textbf{Sizes} & \textbf{\#Examples} & \textbf{copy} & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy} & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy} & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy} & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy} & \textbf{w/o\_copy} & \textbf{Seq2Seq} \\
    \midrule
    1     & 3368  & 60    & 1     & 5     & 101   & 1     & 15    & 124   & 1     & 64    & 138   & 1     & 76    & 170   & 2     & 94 \\
    2 - 5 & 2061  & 9     & 0     & 2     & 21    & 0     & 4     & 60    & 0     & 6     & 73    & 0     & 12    & 95    & 0     & 21 \\
    6 - 10 & 1306  & 156   & 156   & 159   & 156   & 156   & 176   & 160   & 156   & 177   & 161   & 156   & 179   & 161   & 156   & 185 \\
    \midrule
    Total & 6735  & 225   & 157   & 166   & 278   & 157   & 195   & 344   & 157   & 247   & 372   & 157   & 267   & 426   & 158   & 300 \\
          &       & 3.34\%  & 2.33\%  & 2.46\%  & 4.13\%  & 2.33\%  & 2.9\%   & 5.11\%  & 2.33\%  & 3.67\%  & 5.52\%  & 2.33\%  & 3.96\%  & 6.33\%  & 2.35\%  & 4.45\% \\
   \bottomrule
    \end{tabular}
  \label{tab:org-res}
\end{table*}

% % Table generated by Excel2LaTeX from sheet 'Summary_res'
% \begin{table*}[htbp]
% \scriptsize
% \setlength{\tabcolsep}{1pt}
%   \centering
%   \caption{\textbf{\small{Performance of \tool recommending concrete edits
%   %Number of correctly generated patches in top 1/2/5/10/20 patches are shown in the table. In each case, performance of \tool with copy, without copy and also performance of a sequence-2-sequence model are shown.
%   }}}
% %   \caption{\tool performance in actual dataset. Comparison is shown with different variations of \tool and also a sequence-2-sequence model. }
%   %  \begin{tabular}{|c|c||c|c|c|c||c|c|c|c||c|c|c|c||c|c|c|c||c|c|c|c|}
% \begin{tabular}{cc|cccc|cccc|cccc|cccc|cccc}
%     \toprule
%     Edit  &  & \multicolumn{4}{c|}{Top 1}    & \multicolumn{4}{c|}{Top 2}    & \multicolumn{4}{c|}{Top 5}    & \multicolumn{4}{c|}{Top 10}   & \multicolumn{4}{c|}{Top 20} \\

%     Sizes & \#Examples & \tool  & \tool\_w/o\_mask & WO\_COPY & Seq2Seq & BASE  & WO\_MASK & WO\_COPY & Seq2Seq & BASE  & WO\_MASK & WO\_COPY & Seq2Seq & BASE  & WO\_MASK & WO\_COPY & Seq2Seq & BASE  & WO\_MASK & WO\_COPY & Seq2Seq \\
%     \midrule
%     1     & 3368  & 60    & 60    & 1     & 5     & 101   & 101   & 1     & 15    & 125   & 124   & 1     & 64    & 138   & 138   & 1     & 76    & 170   & 170   & 2     & 94 \\
%     \midrule
%     2 - 5 & 2061  & 9     & 9     & 0     & 2     & 21    & 21    & 0     & 4     & 66    & 60    & 0     & 6     & 75    & 73    & 0     & 12    & 100   & 95    & 0     & 21 \\
%     \midrule
%     6 - 10 & 1306  & 156   & 156   & 156   & 159   & 156   & 156   & 156   & 176   & 160   & 160   & 156   & 177   & 161   & 161   & 156   & 179   & 161   & 161   & 156   & 185 \\
%     \midrule
%     11 - 15 & 96    & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 1     & 1     & 0     & 0     & 1     & 1     & 0     & 0 \\
%     \midrule
%     Total & 6831  & 225   & 225   & 157   & 166   & 278   & 278   & 157   & 195   & 351   & 344   & 157   & 247   & 374   & 372   & 157   & 267   & 431   & 426   & 158   & 300 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:org-res}%
% \end{table*}%


==> tables/res.tex <==
% Table generated by Excel2LaTeX from sheet 'summary_result'
\begin{table*}[htbp]
\scriptsize
\setlength{\tabcolsep}{2pt}
  \centering
  \caption{\textbf{\small{Performance of \tool suggesting  edits ~\sk{Is it MAP?, No, it is not, it is number of correct patches. }
  %Number of correctly generated patches in top 1/2/5/10/20 patches are shown in the table. In each case, performance of \tool with copy, without copy and also performance of a sequence-2-sequence model are shown.
  }}}
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc}
    \toprule
      &  & 
    \multicolumn{3}{c|}{Top 1} & 
    \multicolumn{3}{c|}{Top 2} & 
    \multicolumn{3}{c|}{Top 5} &
    \multicolumn{3}{c|}{Top 10} &
    \multicolumn{3}{c}{Top 20} \\
            \cline{3-17}
    \textbf{Edit} &  &  \multicolumn{2}{c}{\tool}  &  &  \multicolumn{2}{c}{\tool}   &   &  \multicolumn{2}{c}{\tool}   &   & \multicolumn{2}{c}{\tool}   &   &  \multicolumn{2}{c}{\tool}   &  \\ \cline{3-4,6-7,9-10,12-13,15-16}
    \textbf{Sizes} & \textbf{\#Examples} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} & \textbf{copy}  & \textbf{w/o\_copy} & \textbf{Seq2Seq} \\
    \midrule
    \multicolumn{17}{c}{\textbf{\textsc{Abstract Edits}}} \\
    \midrule
    1     & 3368  & 586   & 33    & 299   & 785   & 36    & 330   & 1043  & 37    & 460   & 1208  & 41    & 704   & 1358  & 65    & 818 \\
    %\midrule
    2 - 5 & 2061  & 22    & 7     & 1     & 59    & 14    & 3     & 119   & 17    & 27    & 168   & 19    & 39    & 227   & 29    & 87 \\
    %\midrule
    6 - 10 & 1306  & 0     & 2     & 0     & 135   & 164   & 0     & 178   & 166   & 0     & 191   & 166   & 0     & 202   & 168   & 2 \\
    \midrule
   Total & 6735 & 608 & 42 & 300 & 979 & 214 & 333 & 1340 & 220 & 487 & 1567 & 226 & 743 & 1787 & 262 & 907 \\
          &       & 9.00\%  & 0.62\%  & 4.44\%  & 14.50\% & 3.17\%  & 4.93\%  & 19.84\% & 3.26\%  & 7.21\%  & 23.20\% & 3.35\%  & 11.00\% & 26.46\% & 3.88\%  & 13.43\% \\
    \midrule
  \multicolumn{17}{c}{\textbf{\textsc{Concrete Edits}}} \\
    \midrule
    1     & 3368  & 60    & 1     & 5     & 101   & 1     & 15    & 124   & 1     & 64    & 138   & 1     & 76    & 170   & 2     & 94 \\
    2 - 5 & 2061  & 9     & 0     & 2     & 21    & 0     & 4     & 60    & 0     & 6     & 73    & 0     & 12    & 95    & 0     & 21 \\
    6 - 10 & 1306  & 156   & 156   & 159   & 156   & 156   & 176   & 160   & 156   & 177   & 161   & 156   & 179   & 161   & 156   & 185 \\
    \midrule
    Total & 6735  & 225   & 157   & 166   & 278   & 157   & 195   & 344   & 157   & 247   & 372   & 157   & 267   & 426   & 158   & 300 \\
          &       & 3.34\%  & 2.33\%  & 2.46\%  & 4.13\%  & 2.33\%  & 2.9\%   & 5.11\%  & 2.33\%  & 3.67\%  & 5.52\%  & 2.33\%  & 3.96\%  & 6.33\%  & 2.35\%  & 4.45\% \\
   \bottomrule
    \end{tabular}
  \label{tab:res}
\end{table*}


==> tables/tuning.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
 \setlength{\tabcolsep}{3.3pt}
 % \renewcommand*{\arraystretch}{0.9}
  \centering
  \scriptsize
  \caption{\textbf{\small{Evaluating Different Design Choices\vspace{-10pt}}}}
    \begin{tabular}{ccc|ccc}
       \toprule
           \multicolumn{3}{c|}{\textbf{Top 1}} & \multicolumn{3}{c}{\textbf{Top 10}} \\
   \midrule
   \multicolumn{6}{c}{Generating Abstract Patches} \\
   \midrule
     \sts +  & \sts + & Tree2Tree + & \sts +  & \sts +  & Tree2Tree + \\
     %+   & + & + & +   & + & +  \\
    Token &  Token type & Token   & Token &  Token type & Token \\
   %Generation &  & Type &   &  & Type  &  \\
        \midrule
       300  &  444  &  \Red{608}   &   {743}         &  887   & \Red{1567} \\
   \midrule
    \multicolumn{6}{c}{Generating Concrete Patches} \\
   \midrule
     Copy +  & Copy + & No\_copy +  & Copy + & Copy + & No\_copy + \\
    Mask & No\_Mask & No\_Mask & Mask & No\_Mask & No\_Mask \\
    \midrule
           \Red{225}   & \Red{225}   & 157   & \Red{374}   & 372   & 157 \\
    \bottomrule
    \end{tabular}%
  \label{tab:tuning}%
  
  Number marked in \Red{red} reflects best performing choice at that setting.
 
\end{table}







% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%  \setlength{\tabcolsep}{3pt}
%  % \renewcommand*{\arraystretch}{0.9}
%   \centering
%   \scriptsize
%   \caption{\textbf{\small{Evaluating Different Design Choices}}}
%     \begin{tabular}{l|ccc|ccc}
%       \toprule
%           & \multicolumn{3}{c|}{\textbf{Top 1}} & \multicolumn{3}{c}{\textbf{Top 10}} \\
%   \midrule
%     Abstract & \sts   & \sts + & Tree2Tree & \sts   & \sts + & Tree2Tree  \\
%   Patch    & Token &  Token type & model   & Token &  Token type & model \\
%   %Generation &  & Type &   &  & Type  &  \\
%       \cline{2-7}
%       & 300  &  444  &  \Red{608}   &   {743}         &  887   & \Red{1568} \\
%   \midrule
%   \midrule
%     Concrete  & Copy +  & Copy + & No\_copy +  & Copy + & Copy + & No\_copy + \\
%     Patch & Mask & No\_Mask & No\_Mask & Mask & No\_Mask & No\_Mask \\
%     \cline{2-7}
%           & \Red{225}   & \Red{225}   & 157   & \Red{374}   & 372   & 157 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:tuning}%
  
%   Number marked in \Red{red} reflects best performing choice at that setting.
 
% \end{table}








==> tables/type-analysis.tex <==
\begin{center}
\noindent
\begin{minipage}{0.95\linewidth}
% \includegraphics[width=6cm]{images/Change-Categories.pdf}
% \captionof{figure}{Example figure caption (non-floating)}
% \label{fig:examplenf}
%\includegraphics[width=0.95\textwidth]{images/patch_type.pdf}
\includegraphics[width=0.95\textwidth]{images/patch_type1.pdf}
%\captionof{table}{Example Table (non-floating)}
{\scriptsize
 \setlength{\tabcolsep}{1pt}
 %\renewcommand*{\arraystretch}{1}
\begin{tabular}{p{0.25\columnwidth}|p{0.7\columnwidth}}
    \toprule
    \textbf{Change Type} & \textbf{Description} \\
    (\tool-only, both, \sts-only) & (See \Cref{tab:concrete_examples} for examples)\\
    \midrule
    API (354, 204, 38) & Modify API and Method Call (Example-1) \\
    \midrule
    Type (97, 13, 20) & Change of Types (Example-2) \\
    \midrule
    Parameter (48, 5, 33) & Add/delete/modify method parameters (Example-3) \\
    \midrule
    Refactor (37, 7, 28) & Bracketing, variable/method renaming, etc. (Example-4) \\
    \midrule
    Object-Reference (36, 2, 8) & Changes in Object or Class Reference (Example-5)\\
    \midrule
    Statement (28, 0, 27) & Addition, Deletion, Change of statements.  (Example-6) \\
    \midrule
    Inheritance (24, 5, 5) & Add/delete abstract keyword, super() call, @Override  (Example-7) \\
    \midrule
    Exception (23, 4, 0) & Modify related to Catch, Throw, and other exceptions (Example-8)\\
    \midrule
    Other (22, 14, 14) & Conditions, Values, Data-dependency, etc. (Example-9) \\
    \midrule
    Final (21, 24, 42) & Add/delete final keyword (Example-10) \\ 
    \midrule
    Access (10, 12, 6) & Modify Access Type (\eg public, private, protected) (Example-11) \\
    \midrule
    Annotation (1, 0, 13) & Add/delete Nullable  \\%before variable, methods and parameter \\
    \bottomrule
\end{tabular}
}
\captionof{figure}{\textbf{\small Percentage of correct patches per type by \tool, \sts, and both the models at top-10. The table describes each type of change. Left column shows the patch category and number of correctly generated patches in the form (\tool-only, both, \sts-only).}}   
\label{fig:change_category}
\end{minipage} 
\vspace{-1mm}
\end{center}

% \begin{figure*}
% \begin{floatrow}
% \ffigbox{%
%   \includegraphics[width=0.45\textwidth]{images/patch_type1.pdf}
% }{%
%   \caption{\textbf{\small Percentage of correct patches per type by \tool, \sts, and both the models at top-10.}}%
% }
% \capbtabbox{%
% \scriptsize
%   \setlength{\tabcolsep}{0.5pt}
%   \begin{tabular}{l|c|p{3cm}}
%     \toprule
% \textbf{Change Type} & \textbf{\#Correct Patches} & \textbf{Description} \\
%                  & (\tool, both, \sts) & (See \Cref{tab:concrete_examples} for examples)\\
%     \toprule
%     %\midrule
%     API & (354, 204, 38)   & Modify API and Method Call (Example-1) \\
%     %\midrule
%     Type & (97, 13, 20) & Change of Types (Example-2) \\
%     %\midrule
%     Parameter & (48, 5, 33)& Add/delete/modify method parameters (Example-3) \\
%     %\midrule
%     Refactor & (37, 7, 28) & Bracketing, variable/method renaming, etc. (Example-4) \\
%     %\midrule
%     Object Reference & (36, 2, 8) & Changes in Object or Class Reference (Example-5)\\
%     %\midrule
%     Statement Related & (28, 0, 27)& Addition, Deletion, Change of statements.  (Example-6) \\
%     %\midrule
%     Inheritance & (24, 5, 5)& Add/delete abstract keyword, super() call, @Override  (Example-7) \\
%     %\midrule
%     Exception & (23, 4, 0)& Modify related to Catch, Throw, and other exceptions (Example-8)\\
%     %\midrule
%     Other Changes & (22, 14, 14)& Conditions, Values, Data-dependency, etc. (Example-9) \\
%     %\midrule
%     Final & (21, 24, 42)& Add/delete final keyword (Example-10) \\ 
%     %\midrule
%     Access & (10, 12, 6)& Modify Access Type (\eg public, private, protected) (Example-11) \\
%     %\midrule
%     Annotation & (1, 0, 13)& Add/delete Nullable  \\%before variable, methods and parameter \\
%     \bottomrule
% \end{tabular}
% }{%
%   \caption{\textbf{\small Each type of changes in details. 
%   %Left Column of the table shows the patch category and number of correctly generated patches in the form (\tool, both, \sts)
%   }}%
% }
% \end{floatrow}
% \end{figure*}

==> todo.tex <==
%!Tex root=./main.tex

\section{Todos}

\subsection{Experiments}

\begin{itemize}
\item Edit distance for the Patches - { \color{green} Done (Put in the Google Doc, Yet to be dumped in the paper.} \rayb{We need to brainstorm how to present this result.})
\item Case study of edits -  
\item Bug data abstract edits - {\color{red} Training is running, Once the training finishes, I will decode the results. }
\item Bug run test cases
\item case study
\end{itemize}

\subsection{Writing}

\begin{itemize}
\item provide motivating example
\item draw overall architecture
\end{itemize}
